Multiparameter critical quantum metrology with impurity probes

Quantum systems can be used as probes in the context of metrology for enhanced parameter estimation. In particular, the delicacy of critical systems to perturbations can make them ideal sensors. Arguably the simplest realistic probe system is a spin-1/2 impurity, which can be manipulated and measured in-situ when embedded in a fermionic environment. Although entanglement between a single impurity probe and its environment produces nontrivial many-body effects, criticality cannot be leveraged for sensing. Here we introduce instead the two-impurity Kondo (2IK) model as a novel paradigm for critical quantum metrology, and examine the multiparameter estimation scenario at finite temperature. We explore the full metrological phase diagram numerically and obtain exact analytic results near criticality. Enhanced sensitivity to the inter-impurity coupling driving a second-order phase transition is evidenced by diverging quantum Fisher information (QFI) and quantum signal-to-noise ratio (QSNR). However, with uncertainty in both coupling strength and temperature, the multiparameter QFI matrix becomes singular -- even though the parameters to be estimated are independent -- resulting in vanishing QSNRs. We demonstrate that by applying a known control field, the singularity can be removed and measurement sensitivity restored. For general systems, we show that the degradation in the QSNR due to uncertainties in another parameter is controlled by the degree of correlation between the unknown parameters.

==> bibo.tex <==
% ---------------- Bibliography ---------------- %

%2IK
@misc{verma2024measuring,
      title={Measuring two temperatures using a single thermometer}, 
      author={ Verma, H. and  Zych, M. and  Costa, F.},
      year={2024},
      eprint={2403.15186},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Ozgur,
  title = {Low-temperature quantum thermometry boosted by coherence generation},
  author = {Ullah, A. and Naseem, M. T. and M\"ustecapl\ifmmode \imath \else \i \fi{}o\ifmmode \breve{g}\else \u{g}\fi{}lu, O.},
  journal = {Phys. Rev. Res.},
  volume = {5},
  issue = {4},
  pages = {043184},
  numpages = {12},
  year = {2023},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.5.043184},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.043184}
}

@misc{Karol1,
      title={Temperature-Enhanced Critical Quantum Metrology}, 
      author={Ostermann, L. and Gietka, K.},
      year={2024},
      eprint={2312.04176},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{Karol2,
  title = {Combining Critical and Quantum Metrology},
  author = {Hotter, C. and Ritsch, H. and Gietka, K.},
  journal = {Phys. Rev. Lett.},
  volume = {132},
  issue = {6},
  pages = {060801},
  numpages = {8},
  year = {2024},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.132.060801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.132.060801}
}

@article{Saulo,
  title = {In- and out-of-equilibrium quantum metrology with mean-field quantum criticality},
  author = {Wald, S. and Moreira, S. V. and Semi\~ao, F. L.},
  journal = {Phys. Rev. E},
  volume = {101},
  issue = {5},
  pages = {052107},
  numpages = {8},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.101.052107},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.101.052107}
}

@misc{lü2024critical,
      title={Critical quantum metrology robust against dissipation and non-adiabaticity}, 
      author={Lü, J. and Ning, W. and Wu, F. and Zheng, R.H and  Chen, K. and Zhu, X. and  Yang, Z.B and Wu, H.Z and Zheng, S.B},
      year={2024},
      eprint={2403.04475},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@misc{Simone,
      title={Optimality and Noise-Resilience of Critical Quantum Sensing}, 
      author={Alushi, U. and Górecki, W. and Felicetti, S. and Candia, R.D},
      year={2024},
      eprint={2402.15559},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{yu2023criticalityenhanced,
      title={Criticality-Enhanced Precision in Phase Thermometry}, 
      author={ Yu, M. and Nguyen, H. C. and  Nimmrichter, S.},
      year={2023},
      eprint={2311.14578},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{srivastava2023topological,
      title={Topological quantum thermometry}, 
      author={  Srivastava, A.K and  Bhattacharya, U. and  Lewenstein, M. and  Płodzień, M.},
      year={2023},
      eprint={2311.14524},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{candeloro2024dimension,
      title={Dimension matters: precision and incompatibility in multi-parameter quantum estimation models}, 
      author={ Candeloro, A. and  Pazhotan, Z. and Paris, M.G.A},
      year={2024},
      eprint={2403.07106},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{advances_metrology,
  title = {Advances in quantum metrology},
  author = {Giovannetti, V. and Lloyd, S. and Maccone, L.},
  journal = {Nat. Photonics},
  volume = {5},
  issue = {4},
  pages = {222--229},
  numpages = {},
  year = {2011},
  month = {April},
  publisher = {Nature},
  doi = {10.1038/nphoton.2011.35},
  url = {https://doi.org/10.1038/nphoton.2011.35}
}

@article{Metrology_Decoher,
  title = {Qubit metrology and decoherence},
  author = {Shaji, A. and Caves, C. M.},
  journal = {Phys. Rev. A},
  volume = {76},
  issue = {3},
  pages = {032111},
  numpages = {13},
  year = {2007},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.76.032111},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.76.032111}
}

@article{Metrology_Decoher_2,
  title = {Effects of local decoherence on quantum critical metrology},
  author = {Chen, C. and Wang, P. and Liu, R.B.},
  journal = {Phys. Rev. A},
  volume = {104},
  issue = {2},
  pages = {L020601},
  numpages = {5},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.104.L020601},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.104.L020601}
}






@article{bayat2012entanglement,
  title = {Entanglement Probe of Two-Impurity {K}ondo Physics in a Spin Chain},
  author = {Bayat, A. and Bose, S. and Sodano, P. and Johannesson, H.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {6},
  pages = {066403},
  numpages = {5},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.066403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.066403}
}


@article{andrew_entropy_exact,
  title = {Universal low-temperature crossover in two-channel {K}ondo models},
  author = {Mitchell, A. K. and Sela, E.},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {23},
  pages = {235127},
  numpages = {23},
  year = {2012},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.235127},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.85.235127}
}


@article{zarand2006quantum,
  title = {Quantum Criticality in a Double-Quantum-Dot System},
  author = {Zar\'and, G. and Chung, C. H. and Simon, P. and Vojta, M.},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {16},
  pages = {166802},
  numpages = {4},
  year = {2006},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.166802},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.97.166802}
}


@article{bayat2014order,
  title = {An order parameter for impurity systems at quantum criticality},
  author = {Bayat, A. and Johannesson, H. and Bose, S. and Sodano, P.},
  journal = {Nat. Commun.},
  volume = {5},
  issue = {1},
  pages = {3784},
  numpages = {},
  year = {2014},
  month = {May},
  publisher = {Nature},
  doi = {10.1038/ncomms4784},
  url = {https://doi.org/10.1038/ncomms4784}
}

@article{jones1988low,
  title = {Low-Temperature Properties of the Two-Impurity {K}ondo Hamiltonian},
  author = {Jones, B. A. and Varma, C. M. and Wilkins, J. W.},
  journal = {Phys. Rev. Lett.},
  volume = {61},
  issue = {1},
  pages = {125--128},
  numpages = {0},
  year = {1988},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.61.125},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.61.125}
}



@article{mitchell2012two,
  title = {Two-Channel {K}ondo Physics in Two-Impurity {K}ondo Models},
  author = {Mitchell, A. K. and Sela, E. and Logan, D. E.},
  journal = {Phys. Rev. Lett.},
  volume = {108},
  issue = {8},
  pages = {086405},
  numpages = {5},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.108.086405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.086405}
}



@article{affleck1995conformal,
  title = {Conformal-field-theory approach to the two-impurity {K}ondo problem: Comparison with numerical renormalization-group results},
  author = {Affleck, I. and Ludwig, A. W. W. and Jones, B. A.},
  journal = {Phys. Rev. B},
  volume = {52},
  issue = {13},
  pages = {9528--9546},
  numpages = {0},
  year = {1995},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.52.9528},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.52.9528}
}


@article{affleck1992exact,
  title = {Exact critical theory of the two-impurity {K}ondo model},
  author = {Affleck, I. and Ludwig, A. W. W.},
  journal = {Phys. Rev. Lett.},
  volume = {68},
  issue = {7},
  pages = {1046--1049},
  numpages = {0},
  year = {1992},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.68.1046},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.68.1046}
}



@article{sela2011exact,
  title = {Exact Crossover Green Function in the Two-Channel and Two-Impurity {K}ondo Models},
  author = {Sela, E. and Mitchell, A. K. and Fritz, L.},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {14},
  pages = {147202},
  numpages = {4},
  year = {2011},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.147202},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.147202}
}



@article{jeong2001Kondo,
  title={The {K}ondo effect in an artificial quantum dot molecule},
  author={Jeong, H. and Chang, A. M. and Melloch, M. R.},
  journal={Science},
  volume={293},
  number={5538},
  pages={2221--2223},
  year={2001},
  publisher={American Association for the Advancement of Science},
  doi = {10.1126/science.1063182},
  url = {https://www.science.org/doi/abs/10.1126/science.1063182}
}

@article{pouse2023quantum,
  title={Quantum simulation of an exotic quantum critical point in a two-site charge {K}ondo circuit},
  author={Pouse, W. and Peeters, L. and Hsueh, C. L. and Gennser, U. and Cavanna, A. and Kastner, M. A. and Mitchell, A. K. and Goldhaber-Gordon, D.},
  journal={Nat. Phys.},
  volume={19},
  number={4},
  pages={492--499},
  year={2023},
  publisher={Nature Publishing Group UK London},
  doi = {10.1038/s41567-022-01905-4},
  url = {https://doi.org/10.1038/s41567-022-01905-4}
}



@article{bayat2010negativity,
  title = {Negativity as the entanglement measure to probe the {K}ondo regime in the spin-chain {K}ondo model},
  author = {Bayat, A. and Sodano, P. and Bose, S.},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {6},
  pages = {064429},
  numpages = {5},
  year = {2010},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.064429},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.064429}
}




@article{mitchell2014generalized,
  title = {Generalized Wilson chain for solving multichannel quantum impurity problems},
  author = {Mitchell, A. K. and Galpin, M. R. and Wilson-Fletcher, S. and Logan, D. E. and Bulla, R.},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {12},
  pages = {121105},
  numpages = {5},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.121105},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.121105}
}


@article{stadler2016interleaved,
  title = {Interleaved numerical renormalization group as an efficient multiband impurity solver},
  author = {Stadler, K. M. and Mitchell, A. K. and von Delft, J. and Weichselbaum, A.},
  journal = {Phys. Rev. B},
  volume = {93},
  issue = {23},
  pages = {235101},
  numpages = {16},
  year = {2016},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.93.235101},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.93.235101}
}

@article{potok2007observation,
  title={Observation of the two-channel {K}ondo effect},
  author={Potok, R. M and Rau, I. G. and Shtrikman, H. and Oreg, Y. and Goldhaber-Gordon, D.},
  journal={Nature},
  volume={446},
  number={7132},
  pages={167--171},
  year={2007},
  publisher={Nature Publishing Group UK London},
  url = {https://doi.org/10.1038/nature05556},
  doi = {10.1038/nature05556}
}

@article{iftikhar2018tunable,
  title={Tunable quantum criticality and super-ballistic transport in a “charge” {K}ondo circuit},
  author={Iftikhar, Z. and Anthore, A. and Mitchell, A. K. and Parmentier, F. D. and Gennser, U. and Ouerghi, A. and Cavanna, A. and Mora, C. and Simon, P. and Pierre, F.},
  journal={Science},
  volume={360},
  number={6395},
  pages={1315--1320},
  year={2018},
  publisher={American Association for the Advancement of Science},
  url = {https://www.science.org/doi/abs/10.1126/science.aan5592},
  doi = {10.1126/science.aan5592}
}



@article{han2022fractional,
  title = {Fractional Entropy of Multichannel {K}ondo Systems from Conductance-Charge Relations},
  author = {Han, C. and Iftikhar, Z. and Kleeorin, Y. and Anthore, A. and Pierre, F. and Meir, Y. and Mitchell, A. K. and Sela, E.},
  journal = {Phys. Rev. Lett.},
  volume = {128},
  issue = {14},
  pages = {146803},
  numpages = {6},
  year = {2022},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.128.146803},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.146803}
}



@article{child2022entropy,
  title = {Entropy Measurement of a Strongly Coupled Quantum Dot},
  author = {Child, T. and Sheekey, O. and L\"uscher, S. and Fallahi, S. and Gardner, G. C. and Manfra, M. and Mitchell, A. K. and Sela, E. and Kleeorin, Y. and Meir, Y. and Folk, J.},
  journal = {Phys. Rev. Lett.},
  volume = {129},
  issue = {22},
  pages = {227702},
  numpages = {5},
  year = {2022},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.129.227702},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.129.227702}
}



@article{gan1995mapping,
  title = {Mapping the Critical Point of the Two-Impurity {K}ondo Model to a Two-Channel Problem},
  author = {Gan, J.},
  journal = {Phys. Rev. Lett.},
  volume = {74},
  issue = {26},
  pages = {5287--5287},
  numpages = {0},
  year = {1995},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.74.5287},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.74.5287}
}



@article{weichselbaum2007sum,
  title = {Sum-Rule Conserving Spectral Functions from the Numerical Renormalization Group},
  author = {Weichselbaum, A. and von Delft, J.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {7},
  pages = {076402},
  numpages = {4},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.076402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.076402}
}


% ############################################## %

% Multi-Parameter Papers ----------------------- %
% ############################################## %

@article{SLD_Asymptoic_quantum_stat,
  title={On asymptotic quantum statistical inference},
  author={Gill, R. D and Gu{\c{t}}{\u{a}}, M. I.},
  title={From Probability to Statistics and Back: High-Dimensional Models and Processes--A Festschrift in Honor of Jon A. Wellner},
  volume={9},
  pages={105--128},
  year={2013},
  publisher={Institute of Mathematical Statistics},
  doi = {10.1214/12-IMSCOLL909},
}
@article{Compatibility_MP,
  title = {Compatibility in multiparameter quantum metrology},
  author = {Ragy, S. and Jarzyna, M. and Demkowicz-Dobrza\ifmmode \acute{n}\else \'{n}\fi{}ski, R.},
  journal = {Phys. Rev. A},
  volume = {94},
  issue = {5},
  pages = {052108},
  numpages = {11},
  year = {2016},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.94.052108},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.94.052108}
}



@article{jayaprakash1981two,
  title = {Two-Impurity {K}ondo Problem},
  author = {Jayaprakash, C. and Krishna-murthy, H. R. and Wilkins, J. W.},
  journal = {Phys. Rev. Lett.},
  volume = {47},
  issue = {10},
  pages = {737--740},
  numpages = {0},
  year = {1981},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.47.737},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.47.737}
}

@article{Nat_Incomp,
  title={Information complementarity: A new paradigm for decoding quantum incompatibility},
  author={Zhu, H.},
  journal={Sci. Rep.},
  volume={5},
  number={1},
  pages={14317},
  year={2015},
  publisher={Nature},
  doi = {10.1038/srep14317},
  url = {https://doi.org/10.1038/srep14317}
}


@article{heinosaari2016invitation,
  title={An invitation to quantum incompatibility},
  author={Heinosaari, T. and Miyadera, T. and Ziman, M.},
  journal={J. Phys. A Math. Theor. },
  volume={49},
  number={12},
  pages={123001},
  year={2016},
  publisher={IOP Publishing},
  doi = {10.1088/1751-8113/49/12/123001},
}

@article{Liu_2020_QFIM_MPE_Review,
doi = {10.1088/1751-8121/ab5d4d},
url = {https://dx.doi.org/10.1088/1751-8121/ab5d4d},
year = {2019},
month = {dec},
publisher = {IOP Publishing},
volume = {53},
number = {2},
pages = {023001},
author = {Liu, J. and Yuan, H. and Lu, X.M. and Wang, X.},
title = {Quantum Fisher information matrix and multiparameter estimation},
journal = {J. Phys. A Math. Theor. }
}


@article{Safarnak_Simple_QFIM,
  title = {Simple expression for the quantum Fisher information matrix},
  author = {\ifmmode \check{S}\else \v{S}\fi{}afr\'anek, D.},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {4},
  pages = {042322},
  numpages = {6},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.042322},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.042322}
}

@misc{zhou2024limits,
      title={Limits of noisy quantum metrology with restricted quantum controls}, 
      author={Zhou, S.},
      year={2024},
      eprint={2402.18765},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{Yang_2024,
   title={Quantum multiparameter estimation enhanced by a topological phase transition},
   volume={109},
   ISSN={2469-9934},
   url={http://dx.doi.org/10.1103/PhysRevA.109.022604},
   DOI={10.1103/physreva.109.022604},
   number={2},
   journal={Physical Review A},
   publisher={American Physical Society (APS)},
   author={Yang, Y. and Yuan, A. and Li, F.},
   year={2024},
   month=feb }





@article{Mauro_Experimentl_MP_Adapative,
  title = {Experimental multiparameter quantum metrology in adaptive regime},
  author = {Mauro, V. and Valeria, C. and Piacentini, S. and Ceccarelli, F. and Polino, E. and Hoch, F. and Bizzarri, G. and Corrielli, G. and Spagnolo, N. and Osellame, R. and Sciarrino, F.},
  journal = {Phys. Rev. Res.},
  volume = {5},
  issue = {1},
  pages = {013138},
  numpages = {11},
  year = {2023},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.5.013138},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.013138}
}

@article{Lu_HUP_MPE,
  title = {Incorporating {H}eisenberg's Uncertainty Principle into Quantum Multiparameter Estimation},
  author = {Lu, X.M. and Wang, X.},
  journal = {Phys. Rev. Lett.},
  volume = {126},
  issue = {12},
  pages = {120503},
  numpages = {7},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.126.120503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.126.120503}
}

@article{Kaubruegger_Zoller_Baysian_MPE_Vector_Field,
  title = {Optimal and Variational Multiparameter Quantum Metrology and Vector-Field Sensing},
  author = {Kaubruegger, R. and Shankar, A. and Vasilyev, D. V. and Zoller, P.},
  journal = {PRX Quantum},
  volume = {4},
  issue = {2},
  pages = {020333},
  numpages = {21},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.4.020333},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.4.020333}
}

@article{Xia_Incompatible_Limits_MPE,
  title = {Toward incompatible quantum limits on multiparameter estimation},
  author = {Xia, B. and Huang, J. and Li, H. and Wang, H. and Zeng, G.},
  journal = {Nat. Commun.},
  volume = {14},
  issue = {1},
  pages = {1021},
  year = {2023},
  month = {07},
  publisher = {Nature},
  doi = {10.1038/s41467-023-36661-3},
  url = {https://doi.org/10.1038/s41467-023-36661-3}
}

@article{Kull_UTradeoff_MPE,
doi = {10.1088/1751-8121/ab7f67},
url = {https://dx.doi.org/10.1088/1751-8121/ab7f67},
year = {2020},
month = {may},
publisher = {IOP Publishing},
volume = {53},
number = {24},
pages = {244001},
author = {Kull, I and Guérin, P.A and Verstraete, F.},
title = {Uncertainty and trade-offs in quantum multiparameter estimation},
journal = {J. Phys. A Math. Theor. },
}

@article{MGA_Quantumness,
  title={On the quantumness of multiparameter estimation problems for qubit systems},
  author={Razavian, S. and Paris, M.G.A and Genoni, M.G.},
  journal={Entropy},
  volume={22},
  number={11},
  pages={1197},
  year={2020},
  publisher={MDPI}
}


@article{MGA_MPE_Kerr,
  title = {Joint quantum estimation of loss and nonlinearity in driven-dissipative Kerr resonators},
  author = {Asjad, M. and Teklu, B. and Paris, M.G.A.},
  journal = {Phys. Rev. Res.},
  volume = {5},
  issue = {1},
  pages = {013185},
  numpages = {7},
  year = {2023},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.5.013185},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.013185}
}


@article{karki2023z,
  title = {Z3 Parafermion in the Double Charge {K}ondo Model},
  author = {Karki, D. B. and Boulat, E. and Pouse, W. and Goldhaber-Gordon, D. and Mitchell, A. K. and Mora, C.},
  journal = {Phys. Rev. Lett.},
  volume = {130},
  issue = {14},
  pages = {146201},
  numpages = {7},
  year = {2023},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.130.146201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.130.146201}
}


@article{Gessner_Sensitivity_Bounds_MPE,
  title = {Sensitivity Bounds for Multiparameter Quantum Metrology},
  author = {Gessner, M. and Pezz\`e, L. and Smerzi, A.},
  journal = {Phys. Rev. Lett.},
  volume = {121},
  issue = {13},
  pages = {130503},
  numpages = {7},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.121.130503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.121.130503}
}
% ############################################## %
% ############################################## %

# Kondo Physics Papers ------------------------- %
% ############################################## %



@article{bulla2008numerical,
  title = {Numerical renormalization group method for quantum impurity systems},
  author = {Bulla, R. and Costi, T. A. and Pruschke, T.},
  journal = {Rev. Mod. Phys.},
  volume = {80},
  issue = {2},
  pages = {395--450},
  numpages = {0},
  year = {2008},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.80.395},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.80.395}
}

@article{de1934electrical,
  title={The electrical resistance of gold, copper and lead at low temperatures},
  author={De Haas, W. J. and De Boer, J. and Van den Berg, G. J.},
  journal={Physica},
  volume={1},
  number={7-12},
  pages={1115--1124},
  year={1934},
  publisher={Elsevier},
  doi = {https://doi.org/10.1016/S0031-8914(34)80310-2},
  url = {https://www.sciencedirect.com/science/article/pii/S0031891434803102}
}

@article{Kondo1964resistance,
  title={Resistance minimum in dilute magnetic alloys},
  author={Kondo, J.},
  journal={Progress of theoretical physics},
  volume={32},
  issue={1},
  pages={37--49},
  numpages={0},
  year={1964},
  publisher={OUP},
  doi = {10.1143/PTP.32.37},
  url = {https://doi.org/10.1143/PTP.32.37}
}

@article{wilson1975renormalization,
  title = {The renormalization group: Critical phenomena and the {K}ondo problem},
  author = {Wilson, K. G.},
  journal = {Rev. Mod. Phys.},
  volume = {47},
  issue = {4},
  pages = {773--840},
  numpages = {0},
  year = {1975},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.47.773},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.47.773}
}

@article{Murthy_NRG_Anderson,
  title = {Renormalization-group approach to the Anderson model of dilute magnetic alloys. I. Static properties for the symmetric case},
  author = {Krishna-murthy, H. R. and Wilkins, J. W. and Wilson, K. G.},
  journal = {Phys. Rev. B},
  volume = {21},
  issue = {3},
  pages = {1003--1043},
  numpages = {0},
  year = {1980},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.21.1003},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.21.1003}
}

% ############################################## %
% ############################################## %

% General Quantum Metrology -------------------- %
% ############################################## %

@article{1055103,
  author={Yuen, H. and Lax, M.},
  journal={IEEE Transactions on Information Theory}, 
  title={Multiple-parameter quantum estimation and measurement of nonselfadjoint observables}, 
  year={1973},
  volume={19},
  number={6},
  pages={740-750},
  doi={10.1109/TIT.1973.1055103}}

% Kubo mori stuff ------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@inproceedings{Petz2007QuantumIT,
  title={Quantum Information Theory and Quantum Statistics},
  author={Petz, D.},
  year={2007},
  url={https://api.semanticscholar.org/CorpusID:118183706}
}

@article{BALIAN19861,
title = {Dissipation in many-body systems: A geometric approach based on information theory},
journal = {Physics Reports},
volume = {131},
number = {1},
pages = {1-146},
year = {1986},
issn = {0370-1573},
doi = {https://doi.org/10.1016/0370-1573(86)90005-0},
url = {https://www.sciencedirect.com/science/article/pii/0370157386900050},
author = {Balian, R. and Alhassid, Y. and Reinhardt, H.}
}

@article{Masahito,
doi = {10.1088/0305-4470/35/36/302},
url = {https://dx.doi.org/10.1088/0305-4470/35/36/302},
year = {2002},
month = {aug},
publisher = {},
volume = {35},
number = {36},
pages = {7689},
author = {Hayashi, M.},
title = {Two quantum analogues of Fisher information from a large deviation viewpoint of quantum estimation},
journal = {Journal of Physics A: Mathematical and General}}

@article{Petz_Toth,
doi = {10.1007/BF00739578},
url = {https://doi.org/10.1007/BF00739578},
year = {1993},
author = {Petz, D. and Toth, G.},
title = {The Bogoliubov inner product in quantum statistics},
journal = {Letters in Mathematical Physics}
}

@article{toth2014quantum,
  title={Quantum metrology from a quantum information science perspective},
  author={T{\'o}th, G. and Apellaniz, I.},
  journal={J. Phys. A Math. Theor. },
  volume={47},
  number={42},
  pages={424006},
  year={2014},
  publisher={IOP Publishing},
  doi = {10.1088/1751-8113/47/42/424006},
  url = {https://dx.doi.org/10.1088/1751-8113/47/42/424006}
}

@article{Baysian_Berry_PRL,
  title = {Optimal States and Almost Optimal Adaptive Measurements for Quantum Interferometry},
  author = {Berry, D. W. and Wiseman, H. M.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {24},
  pages = {5098--5101},
  numpages = {0},
  year = {2000},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.5098},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.5098}
}

@article{Baysian_2Ref,
  title = {Phase estimation without a priori phase knowledge in the presence of loss},
  author = {Ko\l{}ody\ifmmode \acute{n}\else \'{n}\fi{}ski, J. and Demkowicz-Dobrza\ifmmode \acute{n}\else \'{n}\fi{}ski, R.},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {5},
  pages = {053804},
  numpages = {6},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.053804},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.053804}
}

@article{Baysian_Precsion_Lim,
doi = {10.1088/1367-2630/17/1/013010},
url = {https://dx.doi.org/10.1088/1367-2630/17/1/013010},
year = {2015},
month = {jan},
publisher = {IOP Publishing},
volume = {17},
number = {1},
pages = {013010},
author = {Jarzyna, M. and Demkowicz-Dobrzański, R.},
title = {True precision limits in quantum metrology},
journal = {New Journal of Physics},}



@article{MGA_Magnet,
  title = {Universal Quantum Magnetometry with Spin States at Equilibrium},
  author = {Troiani, F. and Paris, M. G. A.},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {26},
  pages = {260503},
  numpages = {5},
  year = {2018},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.260503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.260503}
}

@Inbook{Mandelstam1991,
author="Mandelstam, L.
and Tamm, Ig.",
editor="Bolotovskii, B. M.
and Frenkel, V. Ya.
and Peierls, R.",
title="The Uncertainty Relation Between Energy and Time in Non-relativistic Quantum Mechanics",
bookTitle="Selected Papers",
year="1991",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="115--123",
abstract="An uncertainty relation between energy and time having a simple physical meaning is rigorously deduced from the principles of quantum mechanics. Some examples of its application are discussed.",
isbn="978-3-642-74626-0",
doi="10.1007/978-3-642-74626-0_8",
url="https://doi.org/10.1007/978-3-642-74626-0_8"
}


@article{Uncert_2,
	title={A unitarity bound on the evolution of nonstationary states},
	author={Fleming, G.  N.},
	journal={Il Nuovo Cimento A},
	volume={16},
	number={2},
	pages={232--240},
	year={1969},
    doi = {10.1007/BF02819419},
    url = {https://doi.org/10.1007/BF02819419}
}

@article{helstrom1969quantum,
	title={Quantum detection and estimation theory},
	author={Helstrom, C. W.},
	journal={J Stat Phy},
	volume={1},
	number={2},
	pages={231--252},
	year={1969},
	publisher={Springer},
    doi = {10.1007/BF01007479},
    url = {https://doi.org/10.1007/BF01007479}
}

@book{Holevo,
	title={Probabilistic and Statistical Aspects of Quantum Theory},
	author={Holevo, A.},
	pages={324},
	year={1982},
	publisher={Edizioni della Normale Pisa},
    doi = {https://doi.org/10.1007/978-88-7642-378-9},
    url = {https://doi.org/10.1007/978-88-7642-378-9}
}


@article{Paris_Quantum_Estimation,
title = {QUANTUM ESTIMATION FOR QUANTUM TECHNOLOGY},
author = {Paris, M. G. A.},
journal = {Int. J. Quantum Inf.},
volume = {07},
number = {supp01},
pages = {125-137},
year = {2009},
doi = {10.1142/S0219749909004839},
url = {https://doi.org/10.1142/S0219749909004839}
}


@book{hewson1997Kondo,
  title={The {K}ondo problem to heavy fermions},
  author={Hewson, A.},
  year={1993},
  publisher={Cambridge Studies in Magnetism, CUP},
  doi = {10.1017/CBO9780511470752},
  url = {https://www.cambridge.org/core/books/{K}ondo-problem-to-heavy-fermions/EDBEDC3F4492DD3EE27E02259935705A}
}

@article{QFI_Ref2,
  title = {Quantum metrology from a quantum information science perspective},
  author = {Tóth, G. and Apellaniz, I.},
  journal = {J. Phys. A.: Math. Theor},
  volume = {47},
  issue = {42},
  pages = {424006},
  numpages = {0},
  year = {2014},
  month = {Oct},
  publisher = {IOP Publishing},
  doi = {10.1088/1751-8113/47/42/424006},
  url = {https://dx.doi.org/10.1088/1751-8113/47/42/424006}
}

@article{Qdv_Quan_Metr,
  title = {Advances in quantum metrology},
  author = {Giovannetti, V. and Lloyd, S. and Maccone, L.},
  journal = {Nat. Photon},
  volume = {5},
  issue = {4},
  year = {2011},
  month = {Apr},
  publisher = {Nature},
  doi = {10.1038/nphoton.2011.35},
  url = {https://doi.org/10.1038/nphoton.2011.35}
}

@article{demkowicz2012elusive,
  title = {The elusive {H}eisenberg limit in quantum-enhanced metrology},
  author = {Demkowicz-Dobrzański, R. and Kołodyński, J. and Guţă, M.},
  journal = {Nat. Commun.},
  volume = {},
  issue = {},
  year = {2012},
  month = {September},
  publisher = {Nature},
  doi = {10.1038/ncomms2067},
  url = {https://doi.org/10.1038/ncomms2067}
}

@article{Preskill_Heisenberg_Lim_Met,
  title = {Achieving the {H}eisenberg limit in quantum metrology using quantum error correction},
  author = {Zhou, S. and Zhang, M. and Preskill, J. and Jiang, L.},
  journal = {Nat. Commun.},
  volume = {9},
  issue = {1},
  year = {2018},
  month = {08},
  publisher = {Nature},
  doi = {10.1038/s41467-017-02510-3},
  url = {https://doi.org/10.1038/s41467-017-02510-3}
}

@article{Napolitano_Super_Heisenberg,
  title={Interaction-based quantum metrology showing scaling beyond the {H}eisenberg limit},
  author={Napolitano, M. and Koschorreck, M. and Dubost, B. and Behbood, N. and Sewell, R.J. and Mitchell, M.W.},
  journal={Nature},
  volume={471},
  number={7339},
  pages={486--489},
  year={2011},
  publisher={Nature},
  doi = {10.1038/nature09778},
  url = {https://doi.org/10.1038/nature09778}
}

@article{Super_Heisen_Experimental,
  title = {Experimental super-{H}eisenberg quantum metrology with indefinite gate order},
  author = {Yin, P. and Zhao, X. and Yang, Y. and Guo, Y. and Zhang, W. H. and Li, G. C. and Han, Y.J. and Liu, B. H. and Xu, J. S. and Chiribella, G. and Chen, G. and Li, C. F. and Guo, G. C.},
  journal = {Nat. Phys.},
  volume = {},
  issue = {},
  year = {2023},
  month = {},
  publisher = {Nature},
  doi = {10.1038/s41567-023-02046-y},
  url = {https://doi.org/10.1038/s41567-023-02046-y}
}

@book{CRB_Book,
	title = {Science from Fisher Information: A Unification},
	doi = {10.1017/CBO9780511616907},
	url = {https://www.cambridge.org/core/books/science-from-fisher-information/ECA32CB301590EF39A88DA9A8E0432B4},
	year = {2004},
	author = {Frieden, B. R.},
	journal = {Cambridge University Press}
}

% Heisenberg Scale stuff
@article{Interfer_Burnett,
  title = {Interferometric detection of optical phase shifts at the {H}eisenberg limit},
  author = {Holland, M. J. and Burnett, K.},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {9},
  pages = {1355--1358},
  numpages = {0},
  year = {1993},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.1355},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.71.1355}
}

@article{Caves_Stat_Dist,
  title = {Statistical distance and the geometry of quantum states},
  author = {Braunstein, S. L. and Caves, Carlton M.},
  journal = {Phys. Rev. Lett.},
  volume = {72},
  issue = {22},
  pages = {3439--3443},
  numpages = {0},
  year = {1994},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.72.3439},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.3439}
}

% ############################################## %
% ############################################## %

% Quantum Thermometry Papers ------------------- %
% ############################################## %
@article{Mihailescu_Thermometry,
  title = {Thermometry of strongly correlated fermionic quantum systems using impurity probes},
  author = {Mihailescu, G. and Campbell, S. and Mitchell, A. K.},
  journal = {Phys. Rev. A},
  volume = {107},
  issue = {4},
  pages = {042614},
  numpages = {16},
  year = {2023},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.107.042614},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.107.042614}
}

@article{BrenesThermometry,
  title = {Multispin probes for thermometry in the strong-coupling regime},
  author = {Brenes, M. and Segal, D.},
  journal = {Phys. Rev. A},
  volume = {108},
  issue = {3},
  pages = {032220},
  numpages = {11},
  year = {2023},
  doi = {10.1103/PhysRevA.108.032220},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.108.032220}
}

@article{Brattegard2023,
         title = {Thermometry by correlated dephasing of impurities in a 1D Fermi gas},
         author = {S. Brattegard and M. T. Mitchison },
         year = {2023},
         eprint = {2307.10132v2},
         archivePrefix = {arXiv},
         primaryClass ={cond-mat.quant-gas}
        }

@article{Landi_Col,
  title = {Bayesian estimation for collisional thermometry},
  author = {Alves, G. O. and Landi, G. T.},
  journal = {Phys. Rev. A},
  volume = {105},
  issue = {1},
  pages = {012212},
  numpages = {10},
  year = {2022},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.105.012212},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.105.012212}
}


@article{Quantum_Limits_Thermo,
  title = {Quantum limits of thermometry},
  author = {Stace, T. M.},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {1},
  pages = {011611},
  numpages = {4},
  year = {2010},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.011611},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.011611}
}

@article{Energy_temp_UR,
  title = {Energy-temperature uncertainty relation in quantum thermodynamics},
  author = {Miller, H. J. D. and Anders, J.},
  journal = {Nat. Commun.},
  volume = {9},
  issue = {1},
  year = {2018},
  month = {Juln},
  publisher = {Nature},
  doi = {10.1038/s41467-018-04536-7},
  url = {https://doi.org/10.1038/s41467-018-04536-7}
}

@article{MitchisonPRL,
  title = {In Situ Thermometry of a Cold Fermi Gas via Dephasing Impurities},
  author = {Mitchison, M. T. and Fogarty, T. and Guarnieri,
  G. and Campbell, S. and Busch, T. and Goold, J.},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  issue = {8},
  pages = {080402},
  numpages = {7},
  year = {2020},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.125.080402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.080402}
}


@article{correa2015individual,
  title = {Individual Quantum Probes for Optimal Thermometry},
  author = {Correa, L. A. and Mehboudi, M. and Adesso, G. and Sanpera, A.},
  journal = {Phys. Rev. Lett.},
  volume = {114},
  issue = {22},
  pages = {220405},
  numpages = {5},
  year = {2015},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.114.220405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.220405}
}


@article{Mehboudi_Thermo_Review,
	title = {Thermometry in the quantum regime: recent theoretical progress},
	doi = {10.1088/1751-8121/ab2828},
	url = {https://doi.org/10.1088/1751-8121/ab2828},
	year = 2019,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {52},
	number = {30},
	pages = {303001},
	author = {Mehboudi, M. and Sanpera, A. and Correa, L. A. },
	journal = {J. Phys. A: Math. Theor}
}


@article{izumida2000two,
  title = {Two-impurity {K}ondo effect in double-quantum-dot systems: Effect of interdot kinetic exchange coupling},
  author = {Izumida, W. and Sakai, O.},
  journal = {Phys. Rev. B},
  volume = {62},
  issue = {15},
  pages = {10260--10267},
  numpages = {0},
  year = {2000},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.62.10260},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.62.10260}
}


@article{van2002electron,
  title = {Electron transport through double quantum dots},
  author = {van der Wiel, W. G. and De Franceschi, S. and Elzerman, J. M. and Fujisawa, T. and Tarucha, S. and Kouwenhoven, L. P.},
  journal = {Rev. Mod. Phys.},
  volume = {75},
  issue = {1},
  pages = {1--22},
  numpages = {0},
  year = {2002},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.75.1},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.75.1}
}


@article{Paris_Landau_Percision_Thermo,
  title = {Achieving the {L}andau bound to precision of quantum thermometry in
  systems with vanishing gap},
	doi = {10.1088/1751-8113/49/3/03lt02},
	url = {https://doi.org/10.1088/1751-8113/49/3/03lt02},
	year = 2015,
	month = {dec},
	publisher = {IOP Publishing},
	volume = {49},
	number = {3},
	pages = {03LT02},
	author = {Paris, M. G. A.},
	journal = {J. Phys. A: Math. Theor.}
}



@article{Campbell_Percision_Thermo_QSL,
  title = {Precision thermometry and the quantum speed limit},
  doi = {10.1088/2058-9565/aaa641},
  url = {https://doi.org/10.1088/2058-9565/aaa641},
  year = 2018,
  month = {feb},
  publisher = {{IOP} Publishing},
  volume = {3},
  number = {2},
  pages = {025002},
  author = {Campbell, S. and Genoni, M. G. and Deffner S. },
  journal = {Quantum Sci. Technol}
}
% ############################################## %
% ############################################## %

% Critical Metrology Papers -------------------- %
% ############################################## %



@article{frerot2018quantum,
  title = {Quantum Critical Metrology},
  author = {Fr\'erot, I. and Roscilde, T.},
  journal = {Phys. Rev. Lett.},
  volume = {121},
  issue = {2},
  pages = {020402},
  numpages = {6},
  year = {2018},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.121.020402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.121.020402}
}


% ############################################## %
% ############################################## %


@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}
@article{macieszczak2016dynamical,
  title = {Dynamical phase transitions as a resource for quantum enhanced metrology},
  author = {Macieszczak, K. and Gu\ifmmode \mbox{\c{t}}\else \c{t}\fi{}\ifmmode \u{a}\else \u{a}\fi{}, M. and Lesanovsky, I. and Garrahan, J. P.},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {2},
  pages = {022103},
  numpages = {10},
  year = {2016},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.022103},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.022103}
}



@article{chu2021dynamic,
  title = {Dynamic Framework for Criticality-Enhanced Quantum Sensing},
  author = {Chu, Y. and Zhang, S. and Yu, B. and Cai, J.},
  journal = {Phys. Rev. Lett.},
  volume = {126},
  issue = {1},
  pages = {010502},
  numpages = {7},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.126.010502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.126.010502}
}

@article{degen2017quantum,
  title = {Quantum sensing},
  author = {Degen, C. L. and Reinhard, F. and Cappellaro, P.},
  journal = {Rev. Mod. Phys.},
  volume = {89},
  issue = {3},
  pages = {035002},
  numpages = {39},
  year = {2017},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.89.035002},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.89.035002}
}


@article{lee2022winding,
title = {Winding number and Zak phase in multi-band SSH models},
journal = {Chinese Journal of Physics},
volume = {78},
pages = {96-110},
year = {2022},
issn = {0577-9073},
doi = {https://doi.org/10.1016/j.cjph.2022.05.007},
url = {https://www.sciencedirect.com/science/article/pii/S0577907322001381},
author = {Chen-Shen Lee and Iao-Fai Io and Hsien-chung Kao},
keywords = {Topological insulator, Bulk edge correspondence, Winding number, The Zak phase},
abstract = {We use multi-band SSH models to demonstrate a prescription for calculating the correct Zak phase and winding number of multi-band systems. We verify our prescription by comparing the resultant winding number of a four-band SSH model with the edge states of a semi-infinite chain which we find by solving the equation of motion. We then also carry out an extensive comparison with the numerical results obtained by solving the matrix eigenvalue problem of finite chains with various number of sites. As a double check of our prescription, we also confirm the bulk edge correspondence in a six-band SSH model. Similar to the usual SSH model, the winding numbers associated to the left and right boundaries in a finite chain may be different if space inversion symmetry is violated in the system. We believe the prescription we propose here may also be applied to other 1D multi-band systems.}
}
@article{alase2016exact,
  title={Exact solution of quadratic fermionic hamiltonians for arbitrary boundary conditions},
  author={Alase, Abhijeet and Cobanera, Emilio and Ortiz, Gerardo and Viola, Lorenza},
  journal={Physical review letters},
  volume={117},
  number={7},
  pages={076804},
  year={2016},
  publisher={APS}
}
@article{Mishra2022integrable,
	doi = {10.1038/s41598-022-17381-y},
  
	url = {https://doi.org/10.1038%2Fs41598-022-17381-y},
  
	year = 2022,
	month = {aug},
  
	publisher = {Springer Science and Business Media {LLC}},
  
	volume = {12},
  
	number = {1},
  
	author = {Mishra, U. and Bayat, A.},
  
	title = {Integrable quantum many-body sensors for {AC} field sensing},
  
	journal = {Sci. Rep.}
}
%%% Elements of Parameter Estimation

@article{PhysRevD.23.357,
  title = {Statistical distance and Hilbert space},
  author = {Wootters, W. K.},
  journal = {Phys. Rev. D},
  volume = {23},
  issue = {2},
  pages = {357--362},
  numpages = {0},
  year = {1981},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.23.357},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.23.357}
}

@article{PhysRevLett.72.3439,
  title = {Statistical distance and the geometry of quantum states},
  author = {Braunstein, Samuel L. and Caves, Carlton M.},
  journal = {Phys. Rev. Lett.},
  volume = {72},
  issue = {22},
  pages = {3439--3443},
  numpages = {0},
  year = {1994},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.72.3439},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.3439}
}


@article{PhysRevA.94.043839,
  title = {Bound states and entanglement generation in waveguide quantum electrodynamics},
  author = {Facchi, Paolo and Kim, M. S. and Pascazio, Saverio and Pepe, Francesco V. and Pomarico, Domenico and Tufarelli, Tommaso},
  journal = {Phys. Rev. A},
  volume = {94},
  issue = {4},
  pages = {043839},
  numpages = {10},
  year = {2016},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.94.043839},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.94.043839}
}

@article{UHLMANN1976273,
title = {The “transition probability” in the state space of a ∗-algebra},
journal = {Reports on Mathematical Physics},
volume = {9},
number = {2},
pages = {273-279},
year = {1976},
issn = {0034-4877},
doi = {https://doi.org/10.1016/0034-4877(76)90060-4},
url = {https://www.sciencedirect.com/science/article/pii/0034487776900604},
author = {A. Uhlmann},
abstract = {Let ω,ϱ be two states of a ∗-algebra and let us consider representations of this algebra R for which ω and ϱ are realized as vector states by vectors x and y. The transition probability P(ω,ϱ) is the spectrum of all the numbers |(x,y)|2 taken over all such realizations. We derive properties of this straightforward generalization of the quantum mechanical transition probability and give, in some important cases, an explicit expression for this quantity.}
}


@Article{Hilgevoord1991,
author={Hilgevoord, Jan
and Uffink, Jos},
title={Uncertainty in prediction and in inference},
journal={Foundations of Physics},
year={1991},
month={Mar},
day={01},
volume={21},
number={3},
pages={323-341},
issn={1572-9516},
doi={10.1007/BF01883638},
url={https://doi.org/10.1007/BF01883638}
}






@book{bengtsson2017geometry,
  title={Geometry of quantum states: an introduction to quantum entanglement},
  author={Bengtsson, Ingemar and {\.Z}yczkowski, Karol},
  year={2017},
  publisher={Cambridge university press}
}

@book{kok2010introduction,
  title={Introduction to optical quantum information processing},
  author={Kok, Pieter and Lovett, Brendon W},
  year={2010},
  publisher={Cambridge university press}
}


@article{einstein-german,
author = {Einstein, A.},
title = {Zur Elektrodynamik bewegter Körper},
journal = {Annalen der Physik},
volume = {322},
number = {10},
pages = {891-921},
year = {1905}
}

@article{PhysRev.59.223,
  title = {Variation of the Rate of Decay of Mesotrons with Momentum},
  author = {Rossi, Bruno and Hall, David B.},
  journal = {Phys. Rev.},
  volume = {59},
  issue = {3},
  pages = {223--228},
  numpages = {0},
  year = {1941},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.59.223},
  url = {https://link.aps.org/doi/10.1103/PhysRev.59.223}
}

@article{Hafele-1,
author = {J. C. Hafele  and Richard E. Keating },
title = {Around-the-World Atomic Clocks: Predicted Relativistic Time Gains},
journal = {Science},
volume = {177},
number = {4044},
pages = {166-168},
year = {1972}}

@article{Hafele-2,
author = {J. C. Hafele  and Richard E. Keating },
title = {Around-the-World Atomic Clocks: Observed Relativistic Time Gains},
journal = {Science},
volume = {177},
number = {4044},
pages = {168-170},
year = {1972}}

@book{Einstein1923-EINTPO,
	author = {Albert Einstein},
	year = {1923},
	publisher = {Dover Publications},
	title = {The Principle of Relativity}
}

@article{Michelson333,
	author = {Michelson, A. A. and Morley, E. W.},
	title = {On the relative motion of the Earth and the luminiferous ether},
	volume = {s3-34},
	number = {203},
	pages = {333--345},
	year = {1887},
	doi = {10.2475/ajs.s3-34.203.333},
	publisher = {American Journal of Science},
	issn = {0002-9599},
	journal = {American Journal of Science}
}

@article{PhysRevLett.116.061102,
  title = {Observation of Gravitational Waves from a Binary Black Hole Merger},
  collaboration = {LIGO Scientific Collaboration and Virgo Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {116},
  issue = {6},
  pages = {061102},
  numpages = {16},
  year = {2016},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.116.061102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.061102}
}

@article{PhysRevLett.13.321,
  title = {Broken Symmetry and the Mass of Gauge Vector Mesons},
  author = {Englert, F. and Brout, R.},
  journal = {Phys. Rev. Lett.},
  volume = {13},
  issue = {9},
  pages = {321--323},
  numpages = {0},
  year = {1964},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.13.321},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.13.321}
}

@article{PhysRevLett.13.508,
  title = {Broken Symmetries and the Masses of Gauge Bosons},
  author = {Higgs, Peter W.},
  journal = {Phys. Rev. Lett.},
  volume = {13},
  issue = {16},
  pages = {508--509},
  numpages = {0},
  year = {1964},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.13.508},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.13.508}
}

@article{PhysRevLett.13.585,
  title = {Global Conservation Laws and Massless Particles},
  author = {Guralnik, G. S. and Hagen, C. R. and Kibble, T. W. B.},
  journal = {Phys. Rev. Lett.},
  volume = {13},
  issue = {20},
  pages = {585--587},
  numpages = {0},
  year = {1964},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.13.585},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.13.585}
}

@Article{TheCMSCollaboration2022,
collaboration={Collaboration, The CMS},
title={A portrait of the Higgs boson by the CMS experiment ten years after the discovery},
journal={Nature},
year={2022},
month={Jul},
day={01},
volume={607},
number={7917},
pages={60-68},
issn={1476-4687},
doi={10.1038/s41586-022-04892-x},
url={https://doi.org/10.1038/s41586-022-04892-x}
}


@article{sidhu2020geometric,
  title={Geometric perspective on quantum parameter estimation},
  author={Sidhu, Jasminder S and Kok, Pieter},
  journal={AVS Quantum Science},
  volume={2},
  number={1},
  pages={014701},
  year={2020},
  publisher={American Vacuum Society}
}

@article{d2000parameter,
  title={Parameter estimation in quantum optics},
  author={D’ariano, G Mauro and Paris, Matteo GA and Sacchi, Massimiliano F},
  journal={Physical Review A},
  volume={62},
  number={2},
  pages={023815},
  year={2000},
  publisher={APS}
}

@article{paris2009quantum,
  title={Quantum estimation for quantum technology},
  author={Paris, Matteo GA},
  journal={International Journal of Quantum Information},
  volume={7},
  number={supp01},
  pages={125--137},
  year={2009},
  publisher={World Scientific}
}

@Book{nla.cat-vn81100,
author = { Cramer, Harald, },
title = { Mathematical methods of statistics / by Harald Cramer },
publisher = { Princeton University Press Princeton },
pages = { xvi, 575 p. ; },
year = { 1946 },
type = { Book },
language = { English },
subjects = { Mathematical statistics. },
life-dates = { 1946 -  },
catalogue-url = { https://nla.gov.au/nla.cat-vn81100 },
}

@Inbook{Rao1992,
author="Rao, C. Radhakrishna",
editor="Kotz, Samuel
and Johnson, Norman L.",
title="Information and the Accuracy Attainable in the Estimation of Statistical Parameters",
bookTitle="Breakthroughs in Statistics: Foundations and Basic Theory",
year="1992",
publisher="Springer New York",
address="New York, NY",
pages="235--247",
isbn="978-1-4612-0919-5",
doi="10.1007/978-1-4612-0919-5_16",
url="https://doi.org/10.1007/978-1-4612-0919-5_16"
}

@Article{Morozova1991,
author={Morozova, E. A.
and Chentsov, N. N.},
title={Markov invariant geometry on manifolds of states},
journal={Journal of Soviet Mathematics},
year={1991},
month={Oct},
day={01},
volume={56},
number={5},
pages={2648-2669},
issn={1573-8795},
doi={10.1007/BF01095975},
url={https://doi.org/10.1007/BF01095975}
}

@article{meyer2021fisher,
  title={Fisher information in noisy intermediate-scale quantum applications},
  author={Meyer, Johannes Jakob},
  journal={Quantum},
  volume={5},
  pages={539},
  year={2021},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@ARTICLE{1055103,  author={Yuen, H. and Lax, M.},  journal={IEEE Transactions on Information Theory},   title={Multiple-parameter quantum estimation and measurement of nonselfadjoint observables},   year={1973},  volume={19},  number={6},  pages={740-750},  doi={10.1109/TIT.1973.1055103}}

@ARTICLE{1055173,  author={Helstrom, C. and Kennedy, R.},  journal={IEEE Transactions on Information Theory},   title={Noncommuting observables in quantum detection and estimation theory},   year={1974},  volume={20},  number={1},  pages={16-24},  doi={10.1109/TIT.1974.1055173}}

@article{tsang2012ziv,
  title={Ziv-Zakai error bounds for quantum parameter estimation},
  author={Tsang, Mankei},
  journal={Physical review letters},
  volume={108},
  number={23},
  pages={230401},
  year={2012},
  publisher={APS}
}

@article{sun2010fisher,
  title = {Fisher information in a quantum-critical environment},
  author = {Sun, Z. and Ma, J. and Lu, X.M. and Wang, X.},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {2},
  pages = {022306},
  numpages = {7},
  year = {2010},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.022306},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.022306}
}


@article{dunningham2004sub,
  title={Sub-shot-noise-limited measurements with Bose-Einstein condensates},
  author={Dunningham, JA and Burnett, K},
  journal={Physical Review A},
  volume={70},
  number={3},
  pages={033601},
  year={2004},
  publisher={APS}
}
@article{lewenstein2007ultracold,
  title={Ultracold atomic gases in optical lattices: mimicking condensed matter physics and beyond},
  author={Lewenstein, Maciej and Sanpera, Anna and Ahufinger, Veronica and Damski, Bogdan and Sen, Aditi and Sen, Ujjwal},
  journal={Advances in Physics},
  volume={56},
  number={2},
  pages={243--379},
  year={2007},
  publisher={Taylor \& Francis}
}
@article{jaksch2005cold,
  title={The cold atom Hubbard toolbox},
  author={Jaksch, Dieter and Zoller, Peter},
  journal={Annals of physics},
  volume={315},
  number={1},
  pages={52--79},
  year={2005},
  publisher={Elsevier}
}
@article{pezze2018quantum,
  title={Quantum metrology with nonclassical states of atomic ensembles},
  author={Pezze, Luca and Smerzi, Augusto and Oberthaler, Markus K and Schmied, Roman and Treutlein, Philipp},
  journal={Reviews of Modern Physics},
  volume={90},
  number={3},
  pages={035005},
  year={2018},
  publisher={APS}
}
@article{gross2010nonlinear,
  title={Nonlinear atom interferometer surpasses classical precision limit},
  author={Gross, Christian and Zibold, Tilman and Nicklas, Eike and Esteve, Jerome and Oberthaler, Markus K},
  journal={Nature},
  volume={464},
  number={7292},
  pages={1165--1169},
  year={2010},
  publisher={Nature Publishing Group}
}
@article{cooper2009scheme,
  title={Scheme for implementing atomic multiport devices},
  author={Cooper, Jessica J and Hallwood, David W and Dunningham, Jacob A},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={42},
  number={10},
  pages={105301},
  year={2009},
  publisher={IOP Publishing}
}
@article{cooling2021quantum,
  title={Quantum-enhanced atomic gyroscope with tunable precision},
  author={Cooling, JP and Dunningham, JA},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={54},
  number={19},
  pages={195502},
  year={2021},
  publisher={IOP Publishing}
}
@article{cooper2010entanglement,
  title={Entanglement-enhanced atomic gyroscope},
  author={Cooper, JJ and Hallwood, DW and Dunningham, JA},
  journal={Physical Review A},
  volume={81},
  number={4},
  pages={043624},
  year={2010},
  publisher={APS}
}
@article{dunningham2002interferometry,
  title={Interferometry below the standard quantum limit with Bose-Einstein condensates},
  author={Dunningham, JA and Burnett, K and Barnett, Stephen M},
  journal={Physical review letters},
  volume={89},
  number={15},
  pages={150401},
  year={2002},
  publisher={APS}
}
@article{jaksch1998cold,
  title={Cold bosonic atoms in optical lattices},
  author={Jaksch, Dieter and Bruder, Christoph and Cirac, Juan Ignacio and Gardiner, Crispin W and Zoller, Peter},
  journal={Physical Review Letters},
  volume={81},
  number={15},
  pages={3108},
  year={1998},
  publisher={APS}
}
@article{lepori2021improving,
  title={Improving producibility estimation for mixed quantum states},
  author={Lepori, Luca and Trombettoni, Andrea and Giuliano, Domenico and Kombe, Johannes and Malo, Jorge Yago and Daley, Andrew J and Smerzi, Augusto and Chiofalo, Maria Luisa},
  journal={arXiv preprint arXiv:2108.03605},
  year={2021}
}

@article{liu2016valid,
  title={Valid lower bound for all estimators in quantum parameter estimation},
  author={Liu, Jing and Yuan, Haidong},
  journal={New Journal of Physics},
  volume={18},
  number={9},
  pages={093009},
  year={2016},
  publisher={IOP Publishing}
}

@article{lu2016quantum,
  title={Quantum Weiss-Weinstein bounds for quantum metrology},
  author={Lu, Xiao-Ming and Tsang, Mankei},
  journal={Quantum Science and Technology},
  volume={1},
  number={1},
  pages={015002},
  year={2016},
  publisher={IOP Publishing}
}

@article{zhang2014quantum,
  title={Quantum metrological bounds for vector parameters},
  author={Zhang, Yu-Ran and Fan, Heng},
  journal={Physical Review A},
  volume={90},
  number={4},
  pages={043818},
  year={2014},
  publisher={APS}
}
@article{chang2022evaluating,
  title={Evaluating the quantum Ziv-Zakai bound in noisy environments},
  author={Chang, Shoukang and Ye, Wei and Rao, Xuan and Zhang, Huan and Luo, Mengmeng and Chen, Yuetao and Gao, Shaoyan and Hu, Liyun},
  journal={arXiv preprint arXiv:2203.11436},
  year={2022}
}
@article{berry2015quantum,
  title={Quantum Bell-Ziv-Zakai bounds and {H}eisenberg limits for waveform estimation},
  author={Berry, Dominic W and Tsang, Mankei and Hall, Michael JW and Wiseman, Howard M},
  journal={Physical Review X},
  volume={5},
  number={3},
  pages={031018},
  year={2015},
  publisher={APS}
}
@article{chang2022evaluating,
  title={Evaluating the quantum Ziv--Zakai bound for phase estimation in noisy environments},
  author={Chang, Shoukang and Ye, Wei and Rao, Xuan and Zhang, Huan and Huang, Liqing and Luo, Mengmeng and Chen, Yuetao and Gao, Shaoyan and Hu, Liyun},
  journal={Optics Express},
  volume={30},
  number={14},
  pages={24207--24221},
  year={2022},
  publisher={Optica Publishing Group}
}
@article{ziv1969some,
  title={Some lower bounds on signal parameter estimation},
  author={Ziv, Jacob and Zakai, Moshe},
  journal={IEEE transactions on Information Theory},
  volume={15},
  number={3},
  pages={386--391},
  year={1969},
  publisher={IEEE}
}
@article{van2007bayesian,
  title={Bayesian bounds for parameter estimation and nonlinear filtering/tracking},
  author={Van Trees, Harry L and Bell, Kristine L},
  journal={AMC},
  volume={10},
  number={12},
  pages={10--1109},
  year={2007}
}

@article{PhysRevLett.72.3439,
  title = {Statistical distance and the geometry of quantum states},
  author = {Braunstein, Samuel L. and Caves, Carlton M.},
  journal = {Phys. Rev. Lett.},
  volume = {72},
  issue = {22},
  pages = {3439--3443},
  numpages = {0},
  year = {1994},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.72.3439},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.3439}
}

@article{albarelli2020perspective,
  title={A perspective on multiparameter quantum metrology: From theoretical tools to applications in quantum imaging},
  author={Albarelli, Francesco and Barbieri, Marco and Genoni, Marco G and Gianani, Ilaria},
  journal={Physics Letters A},
  volume={384},
  number={12},
  pages={126311},
  year={2020},
  publisher={Elsevier}
}

@article{liu2019quantum,
  title={Quantum Fisher information matrix and multiparameter estimation},
  author={Liu, Jing and Yuan, Haidong and Lu, Xiao-Ming and Wang, Xiaoguang},
  journal={J. Phys. A Math. Theor. },
  volume={53},
  number={2},
  pages={023001},
  year={2019},
  publisher={IOP Publishing}
}

@article{rubio2019quantum,
  title={Quantum metrology in the presence of limited data},
  author={Rubio, Jes{\'u}s and Dunningham, Jacob},
  journal={New Journal of Physics},
  volume={21},
  number={4},
  pages={043037},
  year={2019},
  publisher={IOP Publishing}
}

@article{rubio2020bayesian,
  title={Bayesian multiparameter quantum metrology with limited data},
  author={Rubio, Jes{\'u}s and Dunningham, Jacob},
  journal={Physical Review A},
  volume={101},
  number={3},
  pages={032114},
  year={2020},
  publisher={APS}
}

@article{HELSTROM1967101,
title = {Minimum mean-squared error of estimates in quantum statistics},
journal = {Physics Letters A},
volume = {25},
number = {2},
pages = {101-102},
year = {1967},
issn = {0375-9601},
doi = {https://doi.org/10.1016/0375-9601(67)90366-0},
url = {https://www.sciencedirect.com/science/article/pii/0375960167903660},
author = {C.W. Helstrom}}

@book{LeCam-1986,
series = {Springer series in statistics},
publisher = {Springer-Verlag},
isbn = {0387963073},
year = {1986},
title = {Asymptotic methods in statistical decision theory},
address = {New York},
author = {Le Cam, Lucien M.},
keywords = {Mathematical statistics -- Asymptotic theory},
lccn = {^^^86010055^//r87},
}
@article{lucchesi2019many,
  title={Many-body entanglement in short-range interacting fermi gases for metrology},
  author={Lucchesi, Leonardo and Chiofalo, Maria Luisa},
  journal={Physical Review Letters},
  volume={123},
  number={6},
  pages={060406},
  year={2019},
  publisher={APS}
}
@article{jiang2021multiparameter,
  title={Multiparameter quantum metrology using strongly interacting spin systems},
  author={Jiang, Min and Ji, Yunlan and Li, Qing and Liu, Ran and Suter, Dieter and Peng, Xinhua},
  journal={arXiv preprint arXiv:2104.00211},
  year={2021}
}

@article{Hradil-1996,
  title = {Quantum Phase in Interferometry},
  author = {Hradil, Z. and My\ifmmode \check{s}\else \v{s}\fi{}ka, R. and Pe\ifmmode \check{r}\else \v{r}\fi{}ina, J. and Zawisky, M. and Hasegawa, Y. and Rauch, H.},
  journal = {Phys. Rev. Lett.},
  volume = {76},
  issue = {23},
  pages = {4295--4298},
  numpages = {0},
  year = {1996},
  month = {Jun},
  publisher = {American Physical Society},
}

@article{Pezze-2007,
  title = {Phase Detection at the Quantum Limit with Multiphoton Mach-Zehnder Interferometry},
  author = {Pezz\'e, L. and Smerzi, A. and Khoury, G. and Hodelin, J. F. and Bouwmeester, D.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {22},
  pages = {223602},
  numpages = {4},
  year = {2007},
  month = {Nov},
  publisher = {American Physical Society},
}

@article{Olivares-2009,
	year = 2009,
	month = {feb},
	publisher = {{IOP} Publishing},
	volume = {42},
	number = {5},
	pages = {055506},
	author = {Stefano Olivares and Matteo G A Paris},
	title = {Bayesian estimation in homodyne interferometry},
	journal = {Journal of Physics B: Atomic, Molecular and Optical Physics},
}

@book{Holevo:1414149,
      author        = "Holevo, Alexander S",
      title         = "{Probabilistic and Statistical Aspects of Quantum Theory;
                       2nd ed.}",
      publisher     = "Springer",
      address       = "Dordrecht",
      series        = "Publications of the Scuola Normale Superiore. Monographs",
      year          = "2011",
      url           = "https://cds.cern.ch/record/1414149",
      doi           = "10.1007/978-88-7642-378-9",
}

@article{Holevo1977CommutationSO,
  title={Commutation superoperator of a state and its applications to the noncommutative statistics},
  author={Alexander S. Holevo},
  journal={Reports on Mathematical Physics},
  year={1977},
  volume={12},
  pages={251-271}
}

@article{carollo2019quantumness,
  title={On quantumness in multi-parameter quantum estimation},
  author={Carollo, Angelo and Spagnolo, Bernardo and Dubkov, Alexander A and Valenti, Davide},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2019},
  number={9},
  pages={094010},
  year={2019},
  publisher={IOP Publishing}
}

@article{ragy2016compatibility,
  title={Compatibility in multiparameter quantum metrology},
  author={Ragy, Sammy and Jarzyna, Marcin and Demkowicz-Dobrza{\'n}ski, Rafa{\l}},
  journal={Physical Review A},
  volume={94},
  number={5},
  pages={052108},
  year={2016},
  publisher={APS}
}

@article{belliardo2021incompatibility,
  title={Incompatibility in quantum parameter estimation},
  author={Belliardo, Federico and Giovannetti, Vittorio},
  journal={New Journal of Physics},
  volume={23},
  number={6},
  pages={063055},
  year={2021},
  publisher={IOP Publishing}
}

@article{chen2021hierarchical,
  title={Hierarchical incompatibility measures in multi-parameter quantum estimation},
  author={Chen, Hongzhen and Chen, Yu and Yuan, Haidong},
  journal={arXiv preprint arXiv:2109.05807},
  year={2021}
}
%%%%%
@misc{bhattacharyya2023disorderinduced,
      title={Disorder-induced enhancement of precision in quantum metrology}, 
      author={ Bhattacharyya, A. and Ghoshal, A. and  Sen, U.},
      year={2023},
      eprint={2212.08523},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{liu2019quantum,
	doi = {10.1088/1751-8121/ab5d4d},
  
	url = {https://doi.org/10.1088%2F1751-8121%2Fab5d4d},
  
	year = 2019,
	month = {dec},
  
	publisher = {{IOP} Publishing},
  
	volume = {53},
  
	number = {2},
  
	pages = {023001},
  
	author = {Jing Liu and Haidong Yuan and Xiao-Ming Lu and Xiaoguang Wang},
  
	title = {Quantum Fisher information matrix and multiparameter estimation},
  
	journal = {J. Phys. A Math. Theor. }
}

@article{giovannetti2004quantum,
	title={Quantum-enhanced measurements: beating the standard quantum limit},
	author={Giovannetti, V. and Lloyd, S. and Maccone, L.},
	journal={Science},
	volume={306},
	number={5700},
	pages={1330--1336},
	year={2004},
	publisher={American Association for the Advancement of Science},
    doi = {10.1126/science.1104149},
    url = {https://www.science.org/doi/abs/10.1126/science.1104149}
}
@article{simoncini2016computational,
  title={Computational methods for linear matrix equations},
  author={Simoncini, Valeria},
  journal={siam REVIEW},
  volume={58},
  number={3},
  pages={377--441},
  year={2016},
  publisher={SIAM}
}
@article{fiderer2021general,
  title={General expressions for the quantum Fisher information matrix with applications to discrete quantum imaging},
  author={Fiderer, Lukas J and Tufarelli, Tommaso and Piano, Samanta and Adesso, Gerardo},
  journal={PRX Quantum},
  volume={2},
  number={2},
  pages={020308},
  year={2021},
  publisher={APS}
}
@book{laub2005matrix,
  title={Matrix analysis for scientists and engineers},
  author={Laub, Alan J},
  volume={91},
  year={2005},
  publisher={Siam}
}
@article{vsafranek2018simple,
  title={Simple expression for the quantum Fisher information matrix},
  author={{\v{S}}afr{\'a}nek, Dominik},
  journal={Physical Review A},
  volume={97},
  number={4},
  pages={042322},
  year={2018},
  publisher={APS}
}

@article{chen2021effects,
  title={Effects of local decoherence on quantum critical metrology},
  author={Chen, Chong and Wang, Ping and Liu, Ren-Bao},
  journal={Physical Review A},
  volume={104},
  number={2},
  pages={L020601},
  year={2021},
  publisher={APS}
}
@article{gabbrielli2018multipartite,
  title={Multipartite entanglement at finite temperature},
  author={Gabbrielli, Marco and Smerzi, Augusto and Pezz{\`e}, Luca},
  journal={Sci. Rep.},
  volume={8},
  number={1},
  pages={1--18},
  year={2018},
  publisher={Nature Publishing Group}
}
@article{pfeuty1970one,
  title={The one-dimensional Ising model with a transverse field},
  author={Pfeuty, Pierre},
  journal={ANNALS of Physics},
  volume={57},
  number={1},
  pages={79--90},
  year={1970},
  publisher={Elsevier}
}


@article{yang2022super,
  title = {Super-{H}eisenberg scaling in Hamiltonian parameter estimation in the long-range Kitaev chain},
  author = {Yang, J. and Pang, S. and del Campo, A. and Jordan, A. N.},
  journal = {Phys. Rev. Res.},
  volume = {4},
  issue = {1},
  pages = {013133},
  numpages = {15},
  year = {2022},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.4.013133},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.013133}
}


@article{mbeng2020quantum,
  title={The quantum Ising chain for beginners},
  author={Mbeng, Glen Bigan and Russomanno, Angelo and Santoro, Giuseppe E},
  journal={arXiv preprint arXiv:2009.09208},
  volume={59},
  year={2020}
}
@misc{yu2022experimental,
      title={Experimental demonstration of topological bounds in quantum metrology}, 
      author={ Yu, M. and  Li, X. and  Chu, y. and  Mera , B. and  Ünal, F. N.  and  Yang, P. and  Liu, Y. and  Goldman, N. and  Cai, J.},
      year={2022},
      eprint={2206.00546},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{hatano1996localization,
  title={Localization transitions in non-Hermitian quantum mechanics},
  author={Hatano, Naomichi and Nelson, David R},
  journal={Physical review letters},
  volume={77},
  number={3},
  pages={570},
  year={1996},
  publisher={APS}
}
---------------------


@article{koch2022quantum,
  title = {Quantum non-Hermitian topological sensors},
  author = {Koch, F. and Budich, J. C.},
  journal = {Phys. Rev. Res.},
  volume = {4},
  issue = {1},
  pages = {013113},
  numpages = {8},
  year = {2022},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.4.013113},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.013113}
}


@article{anderson1958absence,
  title = {Absence of Diffusion in Certain Random Lattices},
  author = {Anderson, P. W.},
  journal = {Phys. Rev.},
  volume = {109},
  issue = {5},
  pages = {1492--1505},
  numpages = {0},
  year = {1958},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.109.1492},
  url = {https://link.aps.org/doi/10.1103/PhysRev.109.1492}
}
@article{aubry1980analyticity,
author = {Aubry, Serge and André, Gilles},
year = {1980},
month = {01},
pages = {},
title = {Analyticity breaking and Anderson localization in incommensurate lattices},
volume = {3},
journal = {Proceedings, VIII International Colloquium on Group-Theoretical Methods in Physics}
}

@article{gu2010fidelity,
	doi = {10.1142/s0217979210056335},
  
	url = {https://doi.org/10.1142%2Fs0217979210056335},
  
	year = 2010,
	month = {sep},
  
	publisher = {World Scientific Pub Co Pte Ltd},
  
	volume = {24},
  
	number = {23},
  
	pages = {4371--4458},
  
	author = {SHI-JIAN GU},
  
	title = {{FIDELITY} {APPROACH} {TO} {QUANTUM} {PHASE} {TRANSITIONS}
},
  
	journal = {International Journal of Modern Physics B}
}

@article{wei2019fidelity,
  title = {Fidelity susceptibility in one-dimensional disordered lattice models},
  author = {Wei, Bo-Bo},
  journal = {Phys. Rev. A},
  volume = {99},
  issue = {4},
  pages = {042117},
  numpages = {9},
  year = {2019},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.99.042117},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.99.042117}
}

@article{guo2021sensitivity,
  title={Sensitivity of topological edge states in a non-Hermitian dimer chain},
  author={Guo, Zhiwei and Zhang, Tengzhou and Song, Juan and Jiang, Haitao and Chen, Hong},
  journal={Photonics Research},
  volume={9},
  number={4},
  pages={574--582},
  year={2021},
  publisher={Optica Publishing Group}
}
@article{ashida2020non,
  title={Non-hermitian physics},
  author={Ashida, Yuto and Gong, Zongping and Ueda, Masahito},
  journal={Advances in Physics},
  volume={69},
  number={3},
  pages={249--435},
  year={2020},
  publisher={Taylor \& Francis}
}
@article{edvardsson2022sensitivity,
  title={Sensitivity of non-Hermitian systems},
  author={Edvardsson, Elisabet and Ardonne, Eddy},
  journal={Physical Review B},
  volume={106},
  number={11},
  pages={115107},
  year={2022},
  publisher={APS}
}

@article{bergholtz2021exceptional,
  title={Exceptional topology of non-Hermitian systems},
  author={Bergholtz, Emil J and Budich, Jan Carl and Kunst, Flore K},
  journal={Reviews of Modern Physics},
  volume={93},
  number={1},
  pages={015005},
  year={2021},
  publisher={APS}
}

@article{ozdemir2019parity,
  title={Parity--time symmetry and exceptional points in photonics},
  author={{\"O}zdemir, {\c{S}}ahin Kaya and Rotter, Stefan and Nori, Franco and Yang, L},
  journal={Nature materials},
  volume={18},
  number={8},
  pages={783--798},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{miri2019exceptional,
  title={Exceptional points in optics and photonics},
  author={Miri, Mohammad-Ali and Al{\`u}, Andrea},
  journal={Science},
  volume={363},
  number={6422},
  pages={eaar7709},
  year={2019},
  publisher={American Association for the Advancement of Science}
}
----------------------------
@article{mera2022relating,
  title={Relating the topology of Dirac Hamiltonians to quantum geometry: When the quantum metric dictates Chern numbers and winding numbers},
  author={Mera, Bruno and Zhang, Anwei and Goldman, Nathan},
  journal={SciPost Physics},
  volume={12},
  number={1},
  pages={018},
  year={2022}
}


@article{upcoming,
  author={Mukhopadhyay, Chiranjib and Bayat, Abolfazl},
  year ={In preparation}
  }


@article{zanardi2006ground,
  title = {Ground state overlap and quantum phase transitions},
  author = {Zanardi, P. and Paunkovi\ifmmode \acute{c}\else \'{c}\fi{}, N.},
  journal = {Phys. Rev. E},
  volume = {74},
  issue = {3},
  pages = {031123},
  numpages = {6},
  year = {2006},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.74.031123},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.74.031123}
}



@misc{di2022multiparameter,
      title={Multiparameter quantum critical metrology}, 
      author={Di Fresco, G. and Spagnolo, B. and Valenti, D. and Carollo, A.},
      year={2022},
      eprint={2203.12676},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{bakmou2019quantum,
  title={Quantum Fisher information matrix in {H}eisenberg XY model},
  author={Bakmou, L and Slaoui, Abdallah and Daoud, Mohammed and Ahl Laamara, R},
  journal={Quantum Information Processing},
  volume={18},
  number={6},
  pages={1--20},
  year={2019},
  publisher={Springer}
}
@article{roy2008exponentially,
  title={Exponentially enhanced quantum metrology},
  author={Roy, SM and Braunstein, Samuel L},
  journal={Physical review letters},
  volume={100},
  number={22},
  pages={220501},
  year={2008},
  publisher={APS}
}
@misc{yang2024sequential,
      title={Sequential measurements Candeloetry with quantum many-body probes}, 
      author={ Yang, Y. and  Montenegro, V. and  Bayat, A.},
      year={2024},
      eprint={2403.10084},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{cavazzoni2024characterization,
      title={Characterization of partially accessible anisotropic spin chains in the presence of anti-symmetric exchange}, 
      author={ Cavazzoni, S. and  Adani, M. and  Bordone, P. and Paris, M.G.A},
      year={2024},
      eprint={2401.14479},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{bressanini2024multiparameter,
      title={Multi-parameter quantum estimation of single- and two-mode pure Gaussian states}, 
      author={ Bressanini, G. and Genoni, M.G and Kim,M. S. and  Paris, M.G.A},
      year={2024},
      eprint={2403.03919},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{zhao2009singularities,
  title={Singularities in ground-state fidelity and quantum phase transitions for the Kitaev model},
  author={Zhao, Jian-Hui and Zhou, Huan-Qiang},
  journal={Physical Review B},
  volume={80},
  number={1},
  pages={014403},
  year={2009},
  publisher={APS}
}

@article{abasto2008fidelity,
  title = {Fidelity analysis of topological quantum phase transitions},
  author = {Abasto, D. F. and Hamma, A. and Zanardi, P.},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {1},
  pages = {010301},
  numpages = {4},
  year = {2008},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.010301},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.010301}
}


@article{qi2011topological,
  title={Topological insulators and superconductors},
  author={Qi, Xiao-Liang and Zhang, Shou-Cheng},
  journal={Reviews of Modern Physics},
  volume={83},
  number={4},
  pages={1057},
  year={2011},
  publisher={APS}
}
@article{goldman2016topological,
  title={Topological quantum matter with ultracold gases in optical lattices},
  author={Goldman, Nathan and Budich, Jan Carl and Zoller, Peter},
  journal={Nature Physics},
  volume={12},
  number={7},
  pages={639--645},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{morita2006exact,
  title={Exact solutions for the LMG model Hamiltonian based on the Bethe ansatz},
  author={Morita, Hiroyuki and Ohnishi, Hiromasa and da Provid{\^e}ncia, Jo{\~a}o and Nishiyama, Seiya},
  journal={Nuclear Physics B},
  volume={737},
  number={3},
  pages={337--350},
  year={2006},
  publisher={Elsevier}
}

@article{pan1999analytical,
  title={Analytical solutions for the LMG model},
  author={Pan, Feng and Draayer, JP},
  journal={Physics Letters B},
  volume={451},
  number={1-2},
  pages={1--10},
  year={1999},
  publisher={Elsevier}
}
@article{zhang2008topological,
  title={Topological states of quantum matter},
  author={Zhang, Shou-cheng},
  journal={Physics},
  volume={1},
  pages={6},
  year={2008},
  publisher={APS}
}
@book{stanescu2016introduction,
  title={Introduction to topological quantum matter \& quantum computation},
  author={Stanescu, Tudor D},
  year={2016},
  publisher={CRC Press}
}
@article{su1979solitons,
  title={Solitons in polyacetylene},
  author={Su, W\_P and Schrieffer, JR and Heeger, Ao J},
  journal={Physical review letters},
  volume={42},
  number={25},
  pages={1698},
  year={1979},
  publisher={APS}
}
@article{wu2016realization,
  title={Realization of two-dimensional spin-orbit coupling for Bose-Einstein condensates},
  author={Wu, Zhan and Zhang, Long and Sun, Wei and Xu, Xiao-Tian and Wang, Bao-Zong and Ji, Si-Cong and Deng, Youjin and Chen, Shuai and Liu, Xiong-Jun and Pan, Jian-Wei},
  journal={Science},
  volume={354},
  number={6308},
  pages={83--88},
  year={2016},
  publisher={American Association for the Advancement of Science}
}
@article{montenegro2021global,
  title={Global sensing and its impact for quantum many-body probes with criticality},
  author={Montenegro, Victor and Mishra, Utkarsh and Bayat, Abolfazl},
  journal={Physical Review Letters},
  volume={126},
  number={20},
  pages={200501},
  year={2021},
  publisher={APS}
}
@article{gu2009scaling,
  title={Scaling dimension of fidelity susceptibility in quantum phase transitions},
  author={Gu, Shi-Jian and Lin, Hai-Qing},
  journal={EPL (Europhysics Letters)},
  volume={87},
  number={1},
  pages={10003},
  year={2009},
  publisher={IOP Publishing}
}

@article{yang2008fidelity,
  title={Fidelity susceptibility and long-range correlation in the Kitaev honeycomb model},
  author={Yang, Shuo and Gu, Shi-Jian and Sun, Chang-Pu and Lin, Hai-Qing},
  journal={Physical Review A},
  volume={78},
  number={1},
  pages={012304},
  year={2008},
  publisher={APS}
}

@article{gu2010fidelityreview,
  title={Fidelity approach to quantum phase transitions},
  author={Gu, Shi-Jian},
  journal={International Journal of Modern Physics B},
  volume={24},
  number={23},
  pages={4371--4458},
  year={2010},
  publisher={World Scientific}
}
@article{boixo2007generalized,
  title={Generalized limits for single-parameter quantum estimation},
  author={Boixo, Sergio and Flammia, Steven T and Caves, Carlton M and Geremia, John M},
  journal={Physical review letters},
  volume={98},
  number={9},
  pages={090401},
  year={2007},
  publisher={APS}
}
@article{invernizzi2008optimal,
  title={Optimal quantum estimation in spin systems at criticality},
  author={Invernizzi, Carmen and Korbman, Michael and Venuti, Lorenzo Campos and Paris, Matteo GA},
  journal={Physical Review A},
  volume={78},
  number={4},
  pages={042106},
  year={2008},
  publisher={APS}
}


@article{zanardi2008quantum,
  title = {Quantum criticality as a resource for quantum estimation},
  author = {Zanardi, P. and Paris, M. G. A. and Campos Venuti, L.},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {4},
  pages = {042105},
  numpages = {7},
  year = {2008},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.042105},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.042105}
}


@article{gong2008fidelity,
  title={Fidelity, fidelity susceptibility, and von Neumann entropy to characterize the phase diagram of an extended Harper model},
  author={Gong, Longyan and Tong, Peiqing},
  journal={Physical Review B},
  volume={78},
  number={11},
  pages={115114},
  year={2008},
  publisher={APS}
}




@article{rams2018limits,
  title = {At the Limits of Criticality-Based Quantum Metrology: Apparent Super-{H}eisenberg Scaling Revisited},
  author = {Rams, M. M. and Sierant, P. and Dutta, O. and Horodecki, P. and Zakrzewski, J.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {2},
  pages = {021022},
  numpages = {16},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.021022},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.021022}
}



@article{hayashi2022global,
   title={Global {H}eisenberg scaling in noisy and practical phase estimation},
   volume={7},
   ISSN={2058-9565},
   url={http://dx.doi.org/10.1088/2058-9565/ac5d7e},
   DOI={10.1088/2058-9565/ac5d7e},
   number={2},
   journal={Quantum Science and Technology},
   publisher={IOP Publishing},
   author={Hayashi, Masahito and Liu, Zi-Wen and Yuan, Haidong},
   year={2022},
   month={Apr},
   pages={025030} }


@article{salvia2023critical,
  title = {Critical Quantum Metrology Assisted by Real-Time Feedback Control},
  author = {Salvia, R. and Mehboudi, M. and Perarnau-Llobet, M.},
  journal = {Phys. Rev. Lett.},
  volume = {130},
  issue = {24},
  pages = {240803},
  numpages = {7},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.130.240803},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.130.240803}
}

@article{ye2016scaling,
  title={Scaling of quantum Fisher information close to the quantum phase transition in the XY spin chain},
  author={Ye, En-Jia and Hu, Zheng-Da and Wu, Wei},
  journal={Physica B: Condensed Matter},
  volume={502},
  pages={151--154},
  year={2016},
  publisher={Elsevier}
}


@article{liu2021experimental,
  title={Experimental critical quantum metrology with the {H}eisenberg scaling},
  author={Liu, R. and Chen, Y. and Jiang, M. and Yang, X. and Wu, Z. and Li, Y. and Yuan, H. and Peng, X. and Du, J.},
  journal={Npj Quantum Inf.},
  volume={7},
  number={1},
  pages={1--7},
  year={2021},
  publisher={Nature Publishing Group},
  doi = {10.1038/s41534-021-00507-x},
  url = {https://doi.org/10.1038/s41534-021-00507-x}
}




@article{zheng2015probing,
  title={Probing Berezinskii--Kosterlitz--Thouless Phase Transition of Spin-Half XXZ Chain by Quantum Fisher Information},
  author={Zheng, Qiang and Yao, Yao and Xu, Xun-Wei},
  journal={Communications in Theoretical Physics},
  volume={63},
  number={3},
  pages={279},
  year={2015},
  publisher={IOP Publishing}
}
@article{dusuel2004finite,
  title = {Finite-Size Scaling Exponents of the Lipkin-Meshkov-Glick Model},
  author = {Dusuel, S\'ebastien and Vidal, Julien},
  journal = {Phys. Rev. Lett.},
  volume = {93},
  issue = {23},
  pages = {237204},
  numpages = {4},
  year = {2004},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.93.237204},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.93.237204}
}
@article{ma2008reduced,
  title = {Reduced fidelity susceptibility and its finite-size scaling behaviors in the Lipkin-Meshkov-Glick model},
  author = {Ma, Jian and Xu, Lei and Xiong, Heng-Na and Wang, Xiaoguang},
  journal = {Phys. Rev. E},
  volume = {78},
  issue = {5},
  pages = {051126},
  numpages = {7},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.78.051126},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.78.051126}
}



@article{dusuel2005continuous,
  title = {Continuous unitary transformations and finite-size scaling exponents in the Lipkin-Meshkov-Glick model},
  author = {Dusuel, S\'ebastien and Vidal, Julien},
  journal = {Phys. Rev. B},
  volume = {71},
  issue = {22},
  pages = {224420},
  numpages = {18},
  year = {2005},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.71.224420},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.71.224420}
}



@article{salvatori2014quantum,
  title = {Quantum metrology in Lipkin-Meshkov-Glick critical systems},
  author = {Salvatori, G. and Mandarino, A. and Paris, M. G. A.},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {2},
  pages = {022111},
  numpages = {11},
  year = {2014},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.022111},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.022111}
}


@article{liu2015quantum,
  title={Quantum Fisher information in the XXZ model with {D}zyaloshinskii-{M}oriya interaction},
  author={Liu, XM and Du, ZZ and Cheng, WW and Liu, J-M},
  journal={Solid State Communications},
  volume={213},
  pages={24--27},
  year={2015},
  publisher={Elsevier}
}
@article{sachdev1999quantum,
  title={Quantum phase transitions},
  author={Sachdev, Subir},
  journal={Physics world},
  volume={12},
  number={4},
  pages={33},
  year={1999},
  publisher={IOP Publishing}
}

@article{liu2013quantum,
  title={Quantum Fisher information and spin squeezing in the ground state of the XY model},
  author={Liu, Wan-Fang and Ma, Jian and Wang, Xiaoguang},
  journal={J. Phys. A Math. Theor. },
  volume={46},
  number={4},
  pages={045302},
  year={2013},
  publisher={IOP Publishing}
}

@article{ye2018quantum,
  title={Quantum Fisher information and coherence in one-dimensional XY spin models with Dzyaloshinsky-Moriya interactions},
  author={Ye, Biao-Liang and Li, Bo and Wang, Zhi-Xi and Li-Jost, Xianqing and Fei, Shao-Ming},
  journal={SCIENCE CHINA Physics, Mechanics \& Astronomy},
  volume={61},
  number={11},
  pages={1--7},
  year={2018},
  publisher={Springer}
}
@article{ye2020quantum,
  title={Quantum coherence and quantum Fisher information in the XXZ system},
  author={Ye, Biao-Liang and Xue, Li-Yuan and Fang, Yu-Liang and Liu, Sheng and Wu, Qi-Cheng and Zhou, Yan-Hui and Yang, Chui-Ping},
  journal={Physica E: Low-dimensional Systems and Nanostructures},
  volume={115},
  pages={113690},
  year={2020},
  publisher={Elsevier}
}

@article{lambert2019estimates,
  title={Estimates of the quantum Fisher information in the S= 1 antiferromagnetic {H}eisenberg spin chain with uniaxial anisotropy},
  author={Lambert, James and S{\o}rensen, ES},
  journal={Physical Review B},
  volume={99},
  number={4},
  pages={045117},
  year={2019},
  publisher={APS}
}

@article{ozaydin2015quantum,
  title={Quantum Metrology: Surpassing the shot-noise limit with Dzyaloshinskii-Moriya interaction},
  author={Ozaydin, F. and Altintas, A. A.},
  journal={Sci. Rep.},
  volume={5},
  number={1},
  pages={1--6},
  year={2015},
  publisher={Nature Publishing Group},
  doi = {10.1038/srep16360},
  url = {https://doi.org/10.1038/srep16360}
}


@article{fernandez2018Heisenberg,
  title = {{H}eisenberg scaling with classical long-range correlations},
  author = {Fern\'andez-Lorenzo, S. and Dunningham, J. A. and Porras, D.},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {2},
  pages = {023843},
  numpages = {12},
  year = {2018},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.023843},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.023843}
}


@article{skotiniotis2015quantum,
  title={Quantum metrology for the Ising Hamiltonian with transverse magnetic field},
  author={Skotiniotis, Michael and Sekatski, Pavel and D{\"u}r, Wolfgang},
  journal={New Journal of Physics},
  volume={17},
  number={7},
  pages={073032},
  year={2015},
  publisher={IOP Publishing}
}
@article{ozaydin2020parameter,
  title={Parameter estimation with Dzyaloshinskii--Moriya interaction under external magnetic fields},
  author={Ozaydin, Fatih and Altintas, Azmi Ali},
  journal={Optical and Quantum Electronics},
  volume={52},
  number={2},
  pages={1--10},
  year={2020},
  publisher={Springer}
}
@article{mossi2017quantum,
  title={On the quantum spin glass transition on the Bethe lattice},
  author={Mossi, Gianni and Parolini, Tommaso and Pilati, Sebastiano and Scardicchio, Antonello},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2017},
  number={1},
  pages={013102},
  year={2017},
  publisher={IOP Publishing}
}

@article{PhysRevB.82.235114,
  title = {Topological characterization of periodically driven quantum systems},
  author = {Kitagawa, Takuya and Berg, Erez and Rudner, Mark and Demler, Eugene},
  journal = {Phys. Rev. B},
  volume = {82},
  issue = {23},
  pages = {235114},
  numpages = {12},
  year = {2010},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.82.235114},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.82.235114}
}

@article{russomanno2016entanglement,
  title={Entanglement entropy in a periodically driven Ising chain},
  author={Russomanno, Angelo and Santoro, Giuseppe E and Fazio, Rosario},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2016},
  number={7},
  pages={073101},
  year={2016},
  publisher={IOP Publishing}
}

@article{PhysRevLett.102.100403,
  title = {Coherent Control of Dressed Matter Waves},
  author = {Zenesini, Alessandro and Lignier, Hans and Ciampini, Donatella and Morsch, Oliver and Arimondo, Ennio},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {10},
  pages = {100403},
  numpages = {4},
  year = {2009},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.100403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.100403}
}

@article{PhysRevLett.114.140401,
  title = {Many-Body Localization in Periodically Driven Systems},
  author = {Ponte, Pedro and Papi\ifmmode \acute{c}\else \'{c}\fi{}, Z. and Huveneers, Fran\ifmmode \mbox{\c{c}}\else \c{c}\fi{}ois and Abanin, Dmitry A.},
  journal = {Phys. Rev. Lett.},
  volume = {114},
  issue = {14},
  pages = {140401},
  numpages = {5},
  year = {2015},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.114.140401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.140401}
}

@article{ponte2015periodically,
  title={Periodically driven ergodic and many-body localized quantum systems},
  author={Ponte, Pedro and Chandran, Anushya and Papi{\'c}, Z and Abanin, Dmitry A},
  journal={Annals of Physics},
  volume={353},
  pages={196--204},
  year={2015},
  publisher={Elsevier}
}
@article{d2013many,
  title={Many-body energy localization transition in periodically driven systems},
  author={D’Alessio, Luca and Polkovnikov, Anatoli},
  journal={Annals of Physics},
  volume={333},
  pages={19--33},
  year={2013},
  publisher={Elsevier}
}

@article{d2014long,
  title={Long-time behavior of isolated periodically driven interacting lattice systems},
  author={D’Alessio, Luca and Rigol, Marcos},
  journal={Physical Review X},
  volume={4},
  number={4},
  pages={041048},
  year={2014},
  publisher={APS}
}


@article{russomanno2012periodic,
  title={Periodic steady regime and interference in a periodically driven quantum system},
  author={Russomanno, Angelo and Silva, Alessandro and Santoro, Giuseppe E},
  journal={Physical review letters},
  volume={109},
  number={25},
  pages={257201},
  year={2012},
  publisher={APS}
}

@article{lazarides2014periodic,
  title={Periodic thermodynamics of isolated quantum systems},
  author={Lazarides, Achilleas and Das, Arnab and Moessner, Roderich},
  journal={Physical review letters},
  volume={112},
  number={15},
  pages={150401},
  year={2014},
  publisher={APS}
}

@article{grifoni1998driven,
  title={Driven quantum tunneling},
  author={Grifoni, Milena and H{\"a}nggi, Peter},
  journal={Physics Reports},
  volume={304},
  number={5-6},
  pages={229--354},
  year={1998},
  publisher={Elsevier}
}

@article{friedman2019integrable,
  title={Integrable many-body quantum Floquet-Thouless pumps},
  author={Friedman, Aaron J and Gopalakrishnan, Sarang and Vasseur, Romain},
  journal={Physical review letters},
  volume={123},
  number={17},
  pages={170603},
  year={2019},
  publisher={APS}
}

@article{else2016floquet,
  title={Floquet time crystals},
  author={Else, Dominic V and Bauer, Bela and Nayak, Chetan},
  journal={Physical review letters},
  volume={117},
  number={9},
  pages={090402},
  year={2016},
  publisher={APS}
}
@article{peng2021floquet,
  title={Floquet prethermalization in dipolar spin chains},
  author={Peng, Pai and Yin, Chao and Huang, Xiaoyang and Ramanathan, Chandrasekhar and Cappellaro, Paola},
  journal={Nature Physics},
  volume={17},
  number={4},
  pages={444--447},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{yang2019floquet,
  title={Floquet dynamical quantum phase transitions},
  author={Yang, Kai and Zhou, Longwen and Ma, Wenchao and Kong, Xi and Wang, Pengfei and Qin, Xi and Rong, Xing and Wang, Ya and Shi, Fazhan and Gong, Jiangbin and others},
  journal={Physical Review B},
  volume={100},
  number={8},
  pages={085308},
  year={2019},
  publisher={APS}
}



@article{lang2015dynamical,
  title = {Dynamical-Decoupling-Based Quantum Sensing: Floquet Spectroscopy},
  author = {Lang, J. E. and Liu, R. B. and Monteiro, T. S.},
  journal = {Phys. Rev. X},
  volume = {5},
  issue = {4},
  pages = {041016},
  numpages = {12},
  year = {2015},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.5.041016},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.5.041016}
}


@article{wang2022sensing,
  title={Sensing of arbitrary-frequency fields using a quantum mixer},
  author={Wang, Guoqing and Liu, Yi-Xiang and Schloss, Jennifer M and Alsid, Scott T and Braje, Danielle A and Cappellaro, Paola and others},
  journal={Physical Review X},
  volume={12},
  number={2},
  pages={021061},
  year={2022},
  publisher={APS}
}



@article{jiang2022floquet,
  title={Floquet Spin Amplification},
  author={Jiang, Min and Qin, Yushu and Wang, Xin and Wang, Yuanhong and Su, Haowen and Peng, Xinhua and Budker, Dmitry},
  journal={Physical Review Letters},
  volume={128},
  number={23},
  pages={233201},
  year={2022},
  publisher={APS}
}

@article{pang2017optimal,
  title={Optimal adaptive control for quantum metrology with time-dependent Hamiltonians},
  author={Pang, Shengshi and Jordan, Andrew N},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={1--9},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{zhou2020quantum,
  title = {Quantum Metrology with Strongly Interacting Spin Systems},
  author = {Zhou, H. and Choi, J. and Choi, S. and Landig, R. and Douglas, A. M. and Isoya, J. and Jelezko, F. and Onoda, S. and Sumiya, H. and Cappellaro, P. and Knowles, H. S. and Park, H. and Lukin, M. D.},
  journal = {Phys. Rev. X},
  volume = {10},
  issue = {3},
  pages = {031003},
  numpages = {9},
  year = {2020},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.10.031003},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.10.031003}
}




@article{invernizzi2008optimal,
  title={Optimal quantum estimation in spin systems at criticality},
  author={Invernizzi, Carmen and Korbman, Michael and Venuti, Lorenzo Campos and Paris, Matteo GA},
  journal={Physical Review A},
  volume={78},
  number={4},
  pages={042106},
  year={2008},
  publisher={APS}
}
@article{chen2007spin,
  title={Spin-orbital entanglement and quantum phase transitions in a spin-orbital chain with SU (2)$\times$ SU (2) symmetry},
  author={Chen, Yan and Wang, ZD and Li, YQ and Zhang, FC},
  journal={Physical Review B},
  volume={75},
  number={19},
  pages={195113},
  year={2007},
  publisher={APS}
}
@article{damski2013exact,
  title={Exact results for fidelity susceptibility of the quantum Ising model: the interplay between parity, system size, and magnetic field},
  author={Damski, B. and Rams, M. M.},
  journal={J. Phys. A Math. Theor.},
  volume={47},
  number={2},
  pages={025303},
  year={2013},
  publisher={IOP Publishing},
  doi = {10.1088/1751-8113/47/2/025303},
  url = {https://dx.doi.org/10.1088/1751-8113/47/2/025303}
}

%%%%%%%%    Stark localization
@article{van2019bloch,
  title={From Bloch oscillations to many-body localization in clean interacting systems},
  author={van Nieuwenburg, Evert and Baum, Yuval and Refael, Gil},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={19},
  pages={9269--9274},
  year={2019},
  publisher={National Acad Sciences}
}
@article{kolovsky2008interplay,
  title={Interplay between Anderson and Stark localization in 2D lattices},
  author={Kolovsky, Andrey R},
  journal={Physical review letters},
  volume={101},
  number={19},
  pages={190602},
  year={2008},
  publisher={APS}
}

@article{schulz2019stark,
  title = {Stark Many-Body Localization},
  author = {Schulz, M. and Hooley, C. A. and Moessner, R. and Pollmann, F.},
  journal = {Phys. Rev. Lett.},
  volume = {122},
  issue = {4},
  pages = {040606},
  numpages = {5},
  year = {2019},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.122.040606},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.122.040606}
}

@article{chanda2020coexistence,
  title={Coexistence of localized and extended phases: Many-body localization in a harmonic trap},
  author={Chanda, Titas and Yao, Ruixiao and Zakrzewski, Jakub},
  journal={Physical Review Research},
  volume={2},
  number={3},
  pages={032039},
  year={2020},
  publisher={APS}
}
@article{yao2020many,
  title={Many-body localization of bosons in an optical lattice: Dynamics in disorder-free potentials},
  author={Yao, Ruixiao and Zakrzewski, Jakub},
  journal={Physical Review B},
  volume={102},
  number={10},
  pages={104203},
  year={2020},
  publisher={APS}
}




@book{sachdev2011quantum,
  title={Quantum Phase Transitions, Second Edition},
  author={Sachdev, S. and Safari, an O'Reilly Media Company},
  url={https://books.google.com/books?id=j7NKzQEACAAJ},
  year={2011},
  publisher={Cambridge University Press}
}


@article{yu2022quantum,
  title={Quantum Fisher information measurement and verification of the quantum Cram{\'e}r--Rao bound in a solid-state qubit},
  author={Yu, Min and Liu, Yu and Yang, Pengcheng and Gong, Musang and Cao, Qingyun and Zhang, Shaoliang and Liu, Haibin and Heyl, Markus and Ozawa, Tomoki and Goldman, Nathan and others},
  journal={Npj Quantum Inf.},
  volume={8},
  number={1},
  pages={1--8},
  year={2022},
  publisher={Nature Publishing Group}
}

@article{ivanov2021enhanced,
  title={Enhanced Parameter Estimation with Periodically Driven Quantum Probe},
  author={Ivanov, Peter A},
  journal={Entropy},
  volume={23},
  number={10},
  pages={1333},
  year={2021},
  publisher={MDPI}
}




%%%%%%%%% GLOBAL

@article{chan2011laser,
  title={Laser cooling of a nanomechanical oscillator into its quantum ground state},
  author={Chan, Jasper and Alegre, TP and Safavi-Naeini, Amir H and Hill, Jeff T and Krause, Alex and Gr{\"o}blacher, Simon and Aspelmeyer, Markus and Painter, Oskar},
  journal={Nature},
  volume={478},
  number={7367},
  pages={89--92},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{rubio2021global,
  title={Global quantum Candeloetry},
  author={Rubio, Jes{\'u}s and Anders, Janet and Correa, Luis A},
  journal={Physical Review Letters},
  volume={127},
  number={19},
  pages={190402},
  year={2021},
  publisher={APS}
}

@incollection{de2018quantum,
  title={Quantum thermometry},
  author={De Pasquale, Antonella and Stace, Thomas M},
  booktitle={Thermodynamics in the quantum regime},
  pages={503--527},
  year={2018},
  publisher={Springer}
}

@INPROCEEDINGS{1523369,  author={Dauwels, J.},  booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},   title={Computing Bayesian Cramer-Rao bounds},   year={2005},  volume={},  number={},  pages={425-429},  doi={10.1109/ISIT.2005.1523369}}

@article{bj/1186078362,
author = {Richard D. Gill and Boris Y. Levit},
title = {{Applications of the van Trees inequality: a Bayesian Cramér-Rao bound}},
volume = {1},
journal = {Bernoulli},
number = {1-2},
publisher = {Bernoulli Society for Mathematical Statistics and Probability},
pages = {59 -- 79},
keywords = {lower bounds, nonparametric estimation, Parameter estimation, quadratic risk, semi-parametric models},
year = {1995},
doi = {bj/1186078362},
URL = {https://doi.org/}
}

@book{Borovkov1984,
  title={Mathematical Statistics. Parameter Estimation},
  author={Borovkov, A. A.},
  year={1984},
  publisher={Moscow: Nauka}
}

@Article{Inagaki1970,
author={Inagaki, Nobuo},
title={On the limiting distribution of a sequence of estimators with uniformity property},
journal={Annals of the Institute of Statistical Mathematics},
year={1970},
month={Dec},
day={01},
volume={22},
number={1},
pages={1-13},
issn={1572-9052},
doi={10.1007/BF02506318},
url={https://doi.org/10.1007/BF02506318}
}

@Article{Hajek1970,
author={H{\'a}jek, Jaroslav},
title={A characterization of limiting distributions of regular estimates},
journal={Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und Verwandte Gebiete},
year={1970},
month={Dec},
day={01},
volume={14},
number={4},
pages={323-330},
issn={1432-2064},
doi={10.1007/BF00533669},
url={https://doi.org/10.1007/BF00533669}
}


@article{janssen2013convolution,
  title={The convolution theorem of H{\'a}jek and Le Cam-revisited},
  author={Janssen, Arnold and Ostrovski, Vladimir},
  journal={arXiv preprint arXiv:1309.4984},
  year={2013}
}

@book{vantrees1968,
  title={Detection, Estimation and Modulation Theory, Part 1},
  author={van Trees, H. L.},
  year={1968},
  publisher={Wiley \& Sons}
}

@article{KLAASSEN1989267,
title = {The asymptotic spread of estimators},
journal = {Journal of Statistical Planning and Inference},
volume = {23},
number = {3},
pages = {267-285},
year = {1989},
issn = {0378-3758},
doi = {https://doi.org/10.1016/0378-3758(89)90072-4},
url = {https://www.sciencedirect.com/science/article/pii/0378375889900724},
author = {Chris A.J. Klaassen},
keywords = {Estimator, spread, local asymptotic minimax, superefficiency, bounded parameter spaces}}

@ARTICLE{2647,  author={Weinstein, E. and Weiss, A.J.},  journal={IEEE Transactions on Information Theory},   title={A general class of lower bounds in parameter estimation},   year={1988},  volume={34},  number={2},  pages={338-342},  doi={10.1109/18.2647}}

@article{Sandford_2020,
doi = {10.3847/1538-4365/ab9cb0},
url = {https://dx.doi.org/10.3847/1538-4365/ab9cb0},
year = {2020},
month = {jul},
publisher = {The American Astronomical Society},
volume = {249},
number = {2},
pages = {24},
author = {Nathan R. Sandford and Daniel R. Weisz and Yuan-Sen Ting},
title = {Forecasting Chemical Abundance Precision for Extragalactic Stellar Archaeology},
journal = {The Astrophysical Journal Supplement Series}}

@article{refId0,
	author = {{Echeverria, Alex} and {Silva, Jorge F.} and {Mendez, Rene A.} and {Orchard, Marcos}},
	title = {Analysis of the Bayesian Cram\'er-Rao lower bound in astrometry - Studying the impact of prior information in the location of an object},
	DOI= "10.1051/0004-6361/201628220",
	url= "https://doi.org/10.1051/0004-6361/201628220",
	journal = {A\&A},
	year = 2016,
	volume = 594,
	pages = "A111",
}

@article{Kastler,
	author = {{Kastler, Alfred}},
	title = {Quelques suggestions concernant la production optique et la d\'etection optique d'une in\'egalit\'e de population des niveaux de quantifigation spatiale des atomes. Application \`a l'exp\'erience de Stern et Gerlach et \`a la r\'esonance magn\'etique},
	DOI= "10.1051/jphysrad:01950001106025500",
	url= "https://doi.org/10.1051/jphysrad:01950001106025500",
	journal = {J. Phys. Radium},
	year = 1950,
	volume = 11,
	number = 6,
	pages = "255-265",
}

@article{Braun-2018,
  title = {Quantum-enhanced measurements without entanglement},
  author = {Braun, Daniel and Adesso, Gerardo and Benatti, Fabio and Floreanini, Roberto and Marzolino, Ugo and Mitchell, Morgan W. and Pirandola, Stefano},
  journal = {Rev. Mod. Phys.},
  volume = {90},
  issue = {3},
  pages = {035006},
  numpages = {47},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.90.035006},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.90.035006}
}

@article{Okamoto-2017,
  title = {Experimental demonstration of adaptive quantum state estimation for single photonic qubits},
  author = {Okamoto, Ryo and Oyama, Satoshi and Yamagata, Koichi and Fujiwara, Akio and Takeuchi, Shigeki},
  journal = {Phys. Rev. A},
  volume = {96},
  issue = {2},
  pages = {022124},
  numpages = {8},
  year = {2017},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.96.022124},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.96.022124}
}

@article{Okamoto-2012,
  title = {Experimental Demonstration of Adaptive Quantum State Estimation},
  author = {Okamoto, Ryo and Iefuji, Minako and Oyama, Satoshi and Yamagata, Koichi and Imai, Hiroshi and Fujiwara, Akio and Takeuchi, Shigeki},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {13},
  pages = {130404},
  numpages = {5},
  year = {2012},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.130404},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.130404}
}

@article{Fujiwara-2006,
	doi = {10.1088/0305-4470/39/40/014},
	url = {https://doi.org/10.1088/0305-4470/39/40/014},
	year = 2006,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {39},
	number = {40},
	pages = {12489--12504},
	author = {Akio Fujiwara},
	title = {Strong consistency and asymptotic efficiency for adaptive quantum estimation problems},
	journal = {Journal of Physics A: Mathematical and General},
	abstract = {It is shown that for an adaptive quantum estimation scheme based on locally unbiased measurements, the sequence of maximum likelihood estimators is strongly consistent and asymptotically efficient.}
}

@article{Fujiwara-2011,
	doi = {10.1088/1751-8113/44/7/079501},
	url = {https://doi.org/10.1088/1751-8113/44/7/079501},
	year = 2011,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {44},
	number = {7},
	pages = {079501},
	author = {Akio Fujiwara},
	title = {Strong consistency and asymptotic efficiency for adaptive quantum estimation problems},
	journal = {J. Phys. A Math. Theor. },
	abstract = {}
}

@article{Wiseman-1995,
  title = {Adaptive Phase Measurements of Optical Modes: Going Beyond the Marginal $Q$ Distribution},
  author = {Wiseman, H. M.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {25},
  pages = {4587--4590},
  numpages = {0},
  year = {1995},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.4587},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.4587}
}

@article{Armen-2002,
  title = {Adaptive Homodyne Measurement of Optical Phase},
  author = {Armen, Michael A. and Au, John K. and Stockton, John K. and Doherty, Andrew C. and Mabuchi, Hideo},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {13},
  pages = {133602},
  numpages = {4},
  year = {2002},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.133602},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.89.133602}
}

%%%%%%%


@article{gonzalez2022dynamical,
  title={Dynamical quantum phase transition in diamond: Applications in quantum metrology},
  author={Gonz{\'a}lez, Francisco J and Norambuena, Ariel and Coto, Ra{\'u}l},
  journal={Physical Review B},
  volume={106},
  number={1},
  pages={014313},
  year={2022},
  publisher={APS}
}

@article{guan2021identifying,
  title={Identifying and harnessing dynamical phase transitions for quantum-enhanced sensing},
  author={Guan, Qingze and Lewis-Swan, Robert J},
  journal={Physical Review Research},
  volume={3},
  number={3},
  pages={033199},
  year={2021},
  publisher={APS}
}



@article{venuti2007quantum,
  title = {Quantum Critical Scaling of the Geometric Tensors},
  author = {Campos Venuti, L. and Zanardi, P.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {9},
  pages = {095701},
  numpages = {4},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.095701},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.095701}
}


@article{schwandt2009quantum,
  title = {Quantum Monte Carlo Simulations of Fidelity at Magnetic Quantum Phase Transitions},
  author = {Schwandt, D. and Alet, F. and Capponi, S.},
  journal = {Phys. Rev. Lett.},
  volume = {103},
  issue = {17},
  pages = {170501},
  numpages = {4},
  year = {2009},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.103.170501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.170501}
}


@misc{gritsev2009universal,
      title={Universal Dynamics Near Quantum Critical Points}, 
      author={ Gritsev, V. and Polkovnikov, A.},
      year={2010},
      eprint={0910.3692},
      archivePrefix={arXiv},
      primaryClass={cond-mat.stat-mech}
}


@article{gu2008fidelity,
  title = {Fidelity susceptibility, scaling, and universality in quantum critical phenomena},
  author = {Gu, S.J. and Kwok, H.M. and Ning, W.Q. and Lin, H.Q.},
  journal = {Phys. Rev. B},
  volume = {77},
  issue = {24},
  pages = {245109},
  numpages = {5},
  year = {2008},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.77.245109},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.77.245109}
}



@article{greschner2013fidelity,
  title = {Fidelity susceptibility and conductivity of the current in one-dimensional lattice models with open or periodic boundary conditions},
  author = {Greschner, S. and Kolezhuk, A. K. and Vekua, T.},
  journal = {Phys. Rev. B},
  volume = {88},
  issue = {19},
  pages = {195101},
  numpages = {11},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.88.195101},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.88.195101}
}


@article{invernizzi2008optimal,
  title={Optimal quantum estimation in spin systems at criticality},
  author={Invernizzi, Carmen and Korbman, Michael and Venuti, Lorenzo Campos and Paris, Matteo GA},
  journal={Physical Review A},
  volume={78},
  number={4},
  pages={042106},
  year={2008},
  publisher={APS}
}
@article{chen2007spin,
  title={Spin-orbital entanglement and quantum phase transitions in a spin-orbital chain with SU (2)$\times$ SU (2) symmetry},
  author={Chen, Yan and Wang, ZD and Li, YQ and Zhang, FC},
  journal={Physical Review B},
  volume={75},
  number={19},
  pages={195113},
  year={2007},
  publisher={APS}
}

@misc{rodríguez2023strongly,
      title={Strongly coupled fermionic probe for nonequilibrium thermometry}, 
      author={ Rodríguez, R. R. and  Mehboudi, M. and  Horodecki, M. and  Perarnau-Llobet, M.},
      year={2023},
      eprint={2310.14655},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@misc{boeyens2023probe,
      title={Probe thermometry with continuous measurements}, 
      author={ Boeyens, J. and  Annby-Andersson, B. and  Bakhshinezhad, P. and  Haack, G. and  Perarnau-Llobet, M. and  Nimmrichter, S and  Potts, P. P. and  Mehboudi, M.},
      year={2023},
      eprint={2307.13407},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{poo,
  title = {Quantum versus Classical Correlations in Gaussian States},
  author = {Adesso, Gerardo and Datta, Animesh},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {3},
  pages = {030501},
  numpages = {4},
  year = {2010},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.030501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.030501}
}



@article{van2019bloch,
  title={From Bloch oscillations to many-body localization in clean interacting systems},
  author={van Nieuwenburg, Evert and Baum, Yuval and Refael, Gil},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={19},
  pages={9269--9274},
  year={2019},
  publisher={National Acad Sciences}
}
@article{kolovsky2008interplay,
  title={Interplay between Anderson and Stark localization in 2D lattices},
  author={Kolovsky, Andrey R},
  journal={Physical review letters},
  volume={101},
  number={19},
  pages={190602},
  year={2008},
  publisher={APS}
}

@article{chanda2020coexistence,
  title={Coexistence of localized and extended phases: Many-body localization in a harmonic trap},
  author={Chanda, Titas and Yao, Ruixiao and Zakrzewski, Jakub},
  journal={Physical Review Research},
  volume={2},
  number={3},
  pages={032039},
  year={2020},
  publisher={APS}
}
@article{yao2020many,
  title={Many-body localization of bosons in an optical lattice: Dynamics in disorder-free potentials},
  author={Yao, Ruixiao and Zakrzewski, Jakub},
  journal={Physical Review B},
  volume={102},
  number={10},
  pages={104203},
  year={2020},
  publisher={APS}
}
%%%%%%%   ETH
@article{deutsch1991quantum,
  title={Quantum statistical mechanics in a closed system},
  author={Deutsch, Josh M},
  journal={Physical review a},
  volume={43},
  number={4},
  pages={2046},
  year={1991},
  publisher={APS}
}
@article{srednicki1994chaos,
  title={Chaos and quantum thermalization},
  author={Srednicki, Mark},
  journal={Physical review e},
  volume={50},
  number={2},
  pages={888},
  year={1994},
  publisher={APS}
}
@article{rigol2008thermalization,
  title={Thermalization and its mechanism for generic isolated quantum systems},
  author={Rigol, Marcos and Dunjko, Vanja and Olshanii, Maxim},
  journal={Nature},
  volume={452},
  number={7189},
  pages={854--858},
  year={2008},
  publisher={Nature Publishing Group}
}
%%%%%%   Scars
@article{shiraishi2017systematic,
  title={Systematic construction of counterexamples to the eigenstate thermalization hypothesis},
  author={Shiraishi, Naoto and Mori, Takashi},
  journal={Physical review letters},
  volume={119},
  number={3},
  pages={030601},
  year={2017},
  publisher={APS}
}
@article{turner2018weak,
  title={Weak ergodicity breaking from quantum many-body scars},
  author={Turner, Christopher J and Michailidis, Alexios A and Abanin, Dmitry A and Serbyn, Maksym and Papi{\'c}, Zlatko},
  journal={Nature Physics},
  volume={14},
  number={7},
  pages={745--749},
  year={2018},
  publisher={Nature Publishing Group}
}
@article{serbyn2021quantum,
  title={Quantum many-body scars and weak breaking of ergodicity},
  author={Serbyn, Maksym and Abanin, Dmitry A and Papi{\'c}, Zlatko},
  journal={Nature Physics},
  volume={17},
  number={6},
  pages={675--685},
  year={2021},
  publisher={Nature Publishing Group}
}
@article{bernien2017probing,
  title={Probing many-body dynamics on a 51-atom quantum simulator},
  author={Bernien, Hannes and Schwartz, Sylvain and Keesling, Alexander and Levine, Harry and Omran, Ahmed and Pichler, Hannes and Choi, Soonwon and Zibrov, Alexander S and Endres, Manuel and Greiner, Markus and others},
  journal={Nature},
  volume={551},
  number={7682},
  pages={579--584},
  year={2017},
  publisher={Nature Publishing Group}
}
%%%%%%   Scars in sensing
@article{dooley2023entanglement,
  title={Entanglement enhanced metrology with quantum many-body scars},
  author={Dooley, Shane and Pappalardi, Silvia and Goold, John},
  journal={Physical Review B},
  volume={107},
  number={3},
  pages={035123},
  year={2023},
  publisher={APS}
}
@article{desaules2022extensive,
  title={Extensive multipartite entanglement from SU (2) quantum many-body scars},
  author={Desaules, Jean-Yves and Pietracaprina, Francesca and Papi{\'c}, Zlatko and Goold, John and Pappalardi, Silvia},
  journal={Physical Review Letters},
  volume={129},
  number={2},
  pages={020601},
  year={2022},
  publisher={APS}
}
@article{dooley2021robust,
  title={Robust quantum sensing in strongly interacting systems with many-body scars},
  author={Dooley, Shane},
  journal={PRX Quantum},
  volume={2},
  number={2},
  pages={020330},
  year={2021},
  publisher={APS}
}
@article{mark2020eta,
  title={$\eta$-pairing states as true scars in an extended Hubbard model},
  author={Mark, Daniel K and Motrunich, Olexei I},
  journal={Physical Review B},
  volume={102},
  number={7},
  pages={075132},
  year={2020},
  publisher={APS}
}

@article{heyl2018dynamical,
  title={Dynamical quantum phase transitions: a review},
  author={Heyl, Markus},
  journal={Reports on Progress in Physics},
  volume={81},
  number={5},
  pages={054001},
  year={2018},
  publisher={IOP Publishing}
}

@article{jafari2017loschmidt,
  title={Loschmidt echo revivals: Critical and noncritical},
  author={Jafari, R and Johannesson, Henrik},
  journal={Physical review letters},
  volume={118},
  number={1},
  pages={015701},
  year={2017},
  publisher={APS}
}





%%%% DISSIPATIVE SECTION:
@article{arimondo1976nonabsorbing,
  title={Nonabsorbing atomic coherences by coherent two-photon transitions in a three-level optical pumping},
  author={Arimondo, EetGORRIOLS and Orriols, G},
  journal={Nuovo Cimento Lettere},
  volume={17},
  pages={333--338},
  year={1976}
}

@article{alzetta1976experimental,
  title={An experimental method for the observation of rf transitions and laser beat resonances in oriented Na vapour},
  author={Alzetta, GAML and Gozzini, A and Moi, L and Orriols, G},
  journal={Il Nuovo Cimento B (1971-1996)},
  volume={36},
  number={1},
  pages={5--20},
  year={1976},
  publisher={Springer}
}

@article{PhysRevLett.61.826,
  title = {Laser Cooling below the One-Photon Recoil Energy by Velocity-Selective Coherent Population Trapping},
  author = {Aspect, A. and Arimondo, E. and Kaiser, R. and Vansteenkiste, N. and Cohen-Tannoudji, C.},
  journal = {Phys. Rev. Lett.},
  volume = {61},
  issue = {7},
  pages = {826--829},
  numpages = {0},
  year = {1988},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.61.826},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.61.826}
}

@article{myatt2000decoherence,
  title={Decoherence of quantum superpositions through coupling to engineered reservoirs},
  author={Myatt, Christopher J and King, Brian E and Turchette, Quentin A and Sackett, Cass A and Kielpinski, David and Itano, Wayne M and Monroe, CWDJ and Wineland, David J},
  journal={Nature},
  volume={403},
  number={6767},
  pages={269--273},
  year={2000},
  publisher={Nature Publishing Group}
}

@article{PhysRevLett.77.4728,
  title = {Quantum Reservoir Engineering with Laser Cooled Trapped Ions},
  author = {Poyatos, J. F. and Cirac, J. I. and Zoller, P.},
  journal = {Phys. Rev. Lett.},
  volume = {77},
  issue = {23},
  pages = {4728--4731},
  numpages = {0},
  year = {1996},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.77.4728},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.4728}
}

@article{pielawa2010engineering,
  title={Engineering atomic quantum reservoirs for photons},
  author={Pielawa, Susanne and Davidovich, Luiz and Vitali, David and Morigi, Giovanna},
  journal={Physical Review A},
  volume={81},
  number={4},
  pages={043802},
  year={2010},
  publisher={APS}
}

@article{pielawa2007generation,
  title={Generation of Einstein-Podolsky-Rosen-entangled radiation through an atomic reservoir},
  author={Pielawa, Susanne and Morigi, Giovanna and Vitali, David and Davidovich, Luiz},
  journal={Physical review letters},
  volume={98},
  number={24},
  pages={240401},
  year={2007},
  publisher={APS}
}

@incollection{carvalho2001decoherence,
  title={Decoherence, pointer engineering and quantum state protection},
  author={Carvalho, ARR and Milman, P and de Matos Filho, RL and Davidovich, L},
  booktitle={Modern Challenges in Quantum Optics},
  pages={65--79},
  year={2001},
  publisher={Springer}
}

@Article{Verstraete2009,
author={Verstraete, Frank
and Wolf, Michael M.
and Ignacio Cirac, J.},
title={Quantum computation and quantum-state engineering driven by dissipation},
journal={Nature Physics},
year={2009},
month={Sep},
day={01},
volume={5},
number={9},
pages={633-636},
issn={1745-2481},
doi={10.1038/nphys1342},
url={https://doi.org/10.1038/nphys1342}
}

@article{diehl2008quantum,
  title={Quantum states and phases in driven open quantum systems with cold atoms},
  author={Diehl, Sebastian and Micheli, A and Kantian, Adrian and Kraus, B and B{\"u}chler, HP and Zoller, Peter},
  journal={Nature Physics},
  volume={4},
  number={11},
  pages={878--883},
  year={2008},
  publisher={Nature Publishing Group}
}

@article{pastawski2011quantum,
  title={Quantum memories based on engineered dissipation},
  author={Pastawski, Fernando and Clemente, Lucas and Cirac, Juan Ignacio},
  journal={Physical Review A},
  volume={83},
  number={1},
  pages={012304},
  year={2011},
  publisher={APS}
}

@article{barreiro2011open,
  title={An open-system quantum simulator with trapped ions},
  author={Barreiro, Julio T and M{\"u}ller, Markus and Schindler, Philipp and Nigg, Daniel and Monz, Thomas and Chwalla, Michael and Hennrich, Markus and Roos, Christian F and Zoller, Peter and Blatt, Rainer},
  journal={Nature},
  volume={470},
  number={7335},
  pages={486--491},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{goldstein2011environment,
  title={Environment-assisted precision measurement},
  author={Goldstein, Garry and Cappellaro, Paola and Maze, Jero R and Hodges, JS and Jiang, L and S{\o}rensen, Anders S{\o}ndberg and Lukin, MD},
  journal={Physical review letters},
  volume={106},
  number={14},
  pages={140502},
  year={2011},
  publisher={APS}
}

@article{lidar2014review,
  title={Review of Decoherence-Free Subspaces, Noiseless Subsystems, and Dynamical Decoupling},
  author={Lidar, Daniel A},
  journal={Quantum information and computation for chemistry},
  pages={295--354},
  year={2014},
  publisher={Wiley Online Library}
}

@article{lidar1998decoherence,
  title={Decoherence-free subspaces for quantum computation},
  author={Lidar, Daniel A and Chuang, Isaac L and Whaley, K Birgitta},
  journal={Physical Review Letters},
  volume={81},
  number={12},
  pages={2594},
  year={1998},
  publisher={APS}
}

@article{palma1996quantum,
  title={Quantum computers and dissipation},
  author={Palma, G Massimo and Suominen, Kalle-Antti and Ekert, Artur},
  journal={Proceedings of the Royal Society of London. Series A: Mathematical, Physical and Engineering Sciences},
  volume={452},
  number={1946},
  pages={567--584},
  year={1996},
  publisher={The Royal Society London}
}

@article{PhysRevLett.79.1953,
  title = {Preserving Coherence in Quantum Computation by Pairing Quantum Bits},
  author = {Duan, Lu-Ming and Guo, Guang-Can},
  journal = {Phys. Rev. Lett.},
  volume = {79},
  issue = {10},
  pages = {1953--1956},
  numpages = {0},
  year = {1997},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.79.1953},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.79.1953}
}

@book{breuer2002theory,
  title={The theory of open quantum systems},
  author={Breuer, Heinz-Peter and Petruccione, Francesco and others},
  year={2002},
  publisher={Oxford University Press on Demand}
}

@book{orszag2016quantum,
  title={Quantum optics: including noise reduction, trapped ions, quantum trajectories, and decoherence},
  author={Orszag, Miguel},
  year={2016},
  publisher={Springer}
}

@article{zanardi1997dissipative,
  title={Dissipative dynamics in a quantum register},
  author={Zanardi, Paolo},
  journal={Physical Review A},
  volume={56},
  number={6},
  pages={4445},
  year={1997},
  publisher={APS}
}

@article{viola1999dynamical,
  title={Dynamical decoupling of open quantum systems},
  author={Viola, Lorenza and Knill, Emanuel and Lloyd, Seth},
  journal={Physical Review Letters},
  volume={82},
  number={12},
  pages={2417},
  year={1999},
  publisher={APS}
}

@article{khodjasteh2005fault,
  title={Fault-tolerant quantum dynamical decoupling},
  author={Khodjasteh, Kaveh and Lidar, Daniel A},
  journal={Physical review letters},
  volume={95},
  number={18},
  pages={180501},
  year={2005},
  publisher={APS}
}

@article{viola2003robust,
  title={Robust dynamical decoupling of quantum systems with bounded controls},
  author={Viola, Lorenza and Knill, Emanuel},
  journal={Physical Review Letters},
  volume={90},
  number={3},
  pages={037901},
  year={2003},
  publisher={APS}
}

@article{plenio1997quantum,
  title={Quantum error correction in the presence of spontaneous emission},
  author={Plenio, Martin B and Vedral, Vlatko and Knight, Peter L},
  journal={Physical Review A},
  volume={55},
  number={1},
  pages={67},
  year={1997},
  publisher={APS}
}

@article{kjaergaard2020superconducting,
  title={Superconducting qubits: Current state of play},
  author={Kjaergaard, Morten and Schwartz, Mollie E and Braum{\"u}ller, Jochen and Krantz, Philip and Wang, Joel I-J and Gustavsson, Simon and Oliver, William D},
  journal={Annual Review of Condensed Matter Physics},
  volume={11},
  pages={369--395},
  year={2020},
  publisher={Annual Reviews}
}

@article{cantat2020long,
  title={Long-lived circular {R}ydberg states of laser-cooled rubidium atoms in a cryostat},
  author={Cantat-Moltrecht, Tigrane and Corti{\~n}as, Rodrigo and Ravon, Brice and M{\'e}haignerie, Paul and Haroche, Serge and Raimond, Jean-Michel and Favier, Maxime and Brune, Michel and Sayrin, Cl{\'e}ment},
  journal={Physical Review Research},
  volume={2},
  number={2},
  pages={022032},
  year={2020},
  publisher={APS}
}


@Article{Chen2021,
author={Chen, Zijun
and Satzinger, Kevin J.
and Atalaya, Juan
and Korotkov, Alexander N.
and Dunsworth, Andrew
and Sank, Daniel
and Quintana, Chris
and McEwen, Matt
and Barends, Rami
and Klimov, Paul V.
and Hong, Sabrina
and Jones, Cody
and Petukhov, Andre
and Kafri, Dvir
and Demura, Sean
and Burkett, Brian
and Gidney, Craig
and Fowler, Austin G.
and Paler, Alexandru
and Putterman, Harald
and Aleiner, Igor
and Arute, Frank
and Arya, Kunal
and Babbush, Ryan
and Bardin, Joseph C.
and Bengtsson, Andreas
and Bourassa, Alexandre
and Broughton, Michael
and Buckley, Bob B.
and Buell, David A.
and Bushnell, Nicholas
and Chiaro, Benjamin
and Collins, Roberto
and Courtney, William
and Derk, Alan R.
and Eppens, Daniel
and Erickson, Catherine
and Farhi, Edward
and Foxen, Brooks
and Giustina, Marissa
and Greene, Ami
and Gross, Jonathan A.
and Harrigan, Matthew P.
and Harrington, Sean D.
and Hilton, Jeremy
and Ho, Alan
and Huang, Trent
and Huggins, William J.
and Ioffe, L. B.
and Isakov, Sergei V.
and Jeffrey, Evan
and Jiang, Zhang
and Kechedzhi, Kostyantyn
and Kim, Seon
and Kitaev, Alexei
and Kostritsa, Fedor
and Landhuis, David
and Laptev, Pavel
and Lucero, Erik
and Martin, Orion
and McClean, Jarrod R.
and McCourt, Trevor
and Mi, Xiao
and Miao, Kevin C.
and Mohseni, Masoud
and Montazeri, Shirin
and Mruczkiewicz, Wojciech
and Mutus, Josh
and Naaman, Ofer
and Neeley, Matthew
and Neill, Charles
and Newman, Michael
and Niu, Murphy Yuezhen
and O'Brien, Thomas E.
and Opremcak, Alex
and Ostby, Eric
and Pat{\'o}, B{\'a}lint
and Redd, Nicholas
and Roushan, Pedram
and Rubin, Nicholas C.
and Shvarts, Vladimir
and Strain, Doug
and Szalay, Marco
and Trevithick, Matthew D.
and Villalonga, Benjamin
and White, Theodore
and Yao, Z. Jamie
and Yeh, Ping
and Yoo, Juhwan
and Zalcman, Adam
and Neven, Hartmut
and Boixo, Sergio
and Smelyanskiy, Vadim
and Chen, Yu
and Megrant, Anthony
and Kelly, Julian
and AI, Google Quantum},
title={Exponential suppression of bit or phase errors with cyclic error correction},
journal={Nature},
year={2021},
month={Jul},
day={01},
volume={595},
number={7867},
pages={383-387},
issn={1476-4687},
doi={10.1038/s41586-021-03588-y},
url={https://doi.org/10.1038/s41586-021-03588-y}
}



@Article{Herbschleb2019,
author={Herbschleb, E. D.
and Kato, H.
and Maruyama, Y.
and Danjo, T.
and Makino, T.
and Yamasaki, S.
and Ohki, I.
and Hayashi, K.
and Morishita, H.
and Fujiwara, M.
and Mizuochi, N.},
title={Ultra-long coherence times amongst room-temperature solid-state spins},
journal={Nature Communications},
year={2019},
month={Aug},
day={28},
volume={10},
number={1},
pages={3766},
issn={2041-1723},
doi={10.1038/s41467-019-11776-8},
url={https://doi.org/10.1038/s41467-019-11776-8}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%



@article{PhysRevLett.106.090502,
  title = {Dissipative Preparation of Entanglement in Optical Cavities},
  author = {Kastoryano, M. J. and Reiter, F. and S\o{}rensen, A. S.},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {9},
  pages = {090502},
  numpages = {4},
  year = {2011},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.090502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.090502}
}



@article{PhysRevA.82.054103,
  title = {Deterministic creation of stationary entangled states by dissipation},
  author = {Alharbi, A. F. and Ficek, Z.},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {5},
  pages = {054103},
  numpages = {4},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.054103},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.054103}
}


@article{PhysRevA.87.042323,
  title = {Dissipative preparation of large $W$ states in optical cavities},
  author = {Sweke, Ryan and Sinayskiy, Ilya and Petruccione, Francesco},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {4},
  pages = {042323},
  numpages = {17},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.042323},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.042323}
}

@article{li2018dissipation,
  title={Dissipation-induced w state in a {R}ydberg-atom-cavity system},
  author={Li, Dong-Xiao and Shao, Xiao-Qiang and Wu, Jin-Hui and Yi, XX},
  journal={Opt. Lett.},
  volume={43},
  number={8},
  pages={1639--1642},
  year={2018},
  publisher={Optica Publishing Group}
}

@article{PhysRevLett.106.020504,
  title = {Optical Pumping into Many-Body Entanglement},
  author = {Cho, Jaeyoon and Bose, Sougato and Kim, M. S.},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {2},
  pages = {020504},
  numpages = {4},
  year = {2011},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.020504},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.020504}
}

@article{stannigel2012driven,
  title={Driven-dissipative preparation of entangled states in cascaded quantum-optical networks},
  author={Stannigel, Kai and Rabl, Peter and Zoller, Peter},
  journal={New Journal of Physics},
  volume={14},
  number={6},
  pages={063014},
  year={2012},
  publisher={IOP Publishing}
}

@article{PhysRevA.76.022312,
  title = {Non-Markovian entanglement dynamics of quantum continuous variable systems in thermal environments},
  author = {Liu, Kuan-Liang and Goan, Hsi-Sheng},
  journal = {Phys. Rev. A},
  volume = {76},
  issue = {2},
  pages = {022312},
  numpages = {12},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.76.022312},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.76.022312}
}
 @article{statistical1994braunstein,
  title = {Statistical distance and the geometry of quantum states},
  author = {Braunstein, Samuel L. and Caves, Carlton M.},
  journal = {Phys. Rev. Lett.},
  volume = {72},
  issue = {22},
  pages = {3439--3443},
  numpages = {0},
  year = {1994},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.72.3439},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.3439}
}


@article{global2021rubio,
  title = {Global Quantum Thermometry},
  author = {Rubio, Jes\'us and Anders, Janet and Correa, Luis A.},
  journal = {Phys. Rev. Lett.},
  volume = {127},
  issue = {19},
  pages = {190402},
  numpages = {6},
  year = {2021},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.127.190402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.127.190402}
}
@article{garbe2022exponential,
  title = {Exponential time-scaling of estimation precision by reaching a quantum critical point},
  author = {Garbe, L. and Abah, O. and Felicetti, S. and Puebla, R.},
  journal = {Phys. Rev. Res.},
  volume = {4},
  issue = {4},
  pages = {043061},
  numpages = {10},
  year = {2022},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.4.043061},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.043061}
}

@article{tsang2013quantum,
  title = {Quantum transition-edge detectors},
  author = {Tsang, M.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {2},
  pages = {021801},
  numpages = {5},
  year = {2013},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.021801},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.021801}
}
@article{heugel2019quantum,
  title = {Quantum Transducer Using a Parametric Driven-Dissipative Phase Transition},
  author = {Heugel, T. L. and Biondi, M. and Zilberberg, O. and Chitra, R.},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {17},
  pages = {173601},
  numpages = {6},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.173601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.173601}
}

@misc{ilias2023criticalityenhanced,
      title={Criticality-enhanced Electromagnetic Field Sensor with Single Trapped Ions}, 
      author={ Ilias, Y. and  Yang, D. and Huelga, S. F. and Plenio, B. B.},
      year={2023},
      eprint={2304.02050},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{zhu2023rabi,
	doi = {10.1007/s11433-022-2073-9},
  
	url = {https://doi.org/10.1007%2Fs11433-022-2073-9},
  
	year = 2023,
	month = {apr},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {66},
  
	number = {5},
  
	author = {Zhu, X. and Lü, J. J. and Ning, W. and  Wu, F. and Shen, L. T. and Yang, z. B. and Zheng, S. B.},
  
	title = {Criticality-enhanced quantum sensing in the anisotropic quantum Rabi model},
  
	journal = {SCI CHINA PHYS MECH}
}

@article{
gilmore2021quantum,
author = {Kevin A. Gilmore  and Matthew Affolter  and Robert J. Lewis-Swan  and Diego Barberena  and Elena Jordan  and Ana Maria Rey  and John J. Bollinger },
title = {Quantum-enhanced sensing of displacements and electric fields with two-dimensional trapped-ion crystals},
journal = {Science},
volume = {373},
number = {6555},
pages = {673-678},
year = {2021},
doi = {10.1126/science.abi5226},
URL = {https://www.science.org/doi/abs/10.1126/science.abi5226},
eprint = {https://www.science.org/doi/pdf/10.1126/science.abi5226},
abstract = {Harnessing quantum mechanical effects is expected to provide an advantage over classical sensing technology. By entangling the center-of-mass motional state of approximately 150 ions trapped in a two-dimensional Coulomb crystal with their collective spin state, Gilmore et al. demonstrate a quantum-enhanced measurement sensitivity of displacement and electric field. Such enhanced sensitivity could, for instance, find application in probing proposed weak interactions between dark matter and normal matter, as well as enhancing gravitational wave detection. —ISO A quantum-enhanced sensor is developed to detect weak motional displacements and electric fields. Fully controllable ultracold atomic systems are creating opportunities for quantum sensing, yet demonstrating a quantum advantage in useful applications by harnessing entanglement remains a challenging task. Here, we realize a many-body quantum-enhanced sensor to detect displacements and electric fields using a crystal of ~150 trapped ions. The center-of-mass vibrational mode of the crystal serves as a high-Q mechanical oscillator, and the collective electronic spin serves as the measurement device. By entangling the oscillator and collective spin and controlling the coherent dynamics via a many-body echo, a displacement is mapped into a spin rotation while avoiding quantum back-action and thermal noise. We achieve a sensitivity to displacements of 8.8 ± 0.4 decibels below the standard quantum limit and a sensitivity for measuring electric fields of 240 ± 10 nanovolts per meter in 1 second. Feasible improvements should enable the use of trapped ions in searches for dark matter.}}


@Article{ying2022critical,
AUTHOR = {Ying, Z.J. and Felicetti, S. and Liu, G. and Braak, D.},
TITLE = {Critical Quantum Metrology in the Non-Linear Quantum Rabi Model},
JOURNAL = {Entropy},
VOLUME = {24},
YEAR = {2022},
NUMBER = {8},
ARTICLE-NUMBER = {1015},
URL = {https://www.mdpi.com/1099-4300/24/8/1015},
PubMedID = {35892995},
ISSN = {1099-4300},
DOI = {10.3390/e24081015}
}

@article{li2010multi,
  title={Multi-mode entanglement of N harmonic oscillators coupled to a non-Markovian reservoir},
  author={Li, Gao-xiang and Sun, Li-hui and Ficek, Zbigniew},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={43},
  number={13},
  pages={135501},
  year={2010},
  publisher={IOP Publishing}
}



@article{PhysRevA.90.062322,
  title = {Steady entanglement in bosonic dissipative networks},
  author = {de Moraes Neto, G. D. and Rosado, W. and Prado, F. O. and Moussa, M. H. Y.},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {6},
  pages = {062322},
  numpages = {6},
  year = {2014},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.062322},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.062322}
}

@article{chu2023strong,
  title = {Strong Quantum Metrological Limit from Many-Body Physics},
  author = {Chu, Y. and Li, X. and Cai, J.},
  journal = {Phys. Rev. Lett.},
  volume = {130},
  issue = {17},
  pages = {170801},
  numpages = {7},
  year = {2023},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.130.170801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.130.170801}
}





@article{de2017steady,
  title={Steady many-body entanglements in dissipative systems},
  author={de Moraes Neto, GD and Teizen, VF and Montenegro, V and Vernek, E},
  journal={Physical Review A},
  volume={96},
  number={6},
  pages={062313},
  year={2017},
  publisher={APS}
}

@article{kacprowicz2010experimental,
  title={Experimental quantum-enhanced estimation of a lossy phase shift},
  author={Kacprowicz, M and Demkowicz-Dobrza{\'n}ski, R and Wasilewski, W and Banaszek, K and Walmsley, IA},
  journal={Nature Photonics},
  volume={4},
  number={6},
  pages={357--360},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{kolodynski2010phase,
  title={Phase estimation without a priori knowledge in the presence of loss},
  author={Kolodynski, Jan and Demkowicz-Dobrzanski, Rafal},
  journal={arXiv preprint arXiv:1006.0734},
  year={2010}
}

@article{knysh2011scaling,
  title={Scaling laws for precision in quantum interferometry and the bifurcation landscape of the optimal state},
  author={Knysh, Sergey and Smelyanskiy, Vadim N and Durkin, Gabriel A},
  journal={Physical Review A},
  volume={83},
  number={2},
  pages={021804},
  year={2011},
  publisher={APS}
}

@article{escher2011general,
  title={General framework for estimating the ultimate precision limit in noisy quantum-enhanced metrology},
  author={Escher, BM and de Matos Filho, RL and Davidovich, Luiz},
  journal={Nature Physics},
  volume={7},
  number={5},
  pages={406--411},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{PhysRevA.88.042112,
  title = {Quantum limit for the measurement of a classical force coupled to a noisy quantum-mechanical oscillator},
  author = {Latune, C. L. and Escher, B. M. and de Matos Filho, R. L. and Davidovich, L.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {4},
  pages = {042112},
  numpages = {15},
  year = {2013},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.042112},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.042112}
}

@article{escher2012quantum,
  title={Quantum metrological limits via a variational approach},
  author={Escher, BM and Davidovich, L and Zagury, N and de Matos Filho, RL},
  journal={Physical review letters},
  volume={109},
  number={19},
  pages={190404},
  year={2012},
  publisher={APS}
}


@article{plenio2016sensing,
  title={Sensing in the presence of an observed environment},
  author={Plenio, Martin B and Huelga, Susana F},
  journal={Physical Review A},
  volume={93},
  number={3},
  pages={032123},
  year={2016},
  publisher={APS}
}

@article{albarelli2018restoring,
  title={Restoring {H}eisenberg scaling in noisy quantum metrology by monitoring the environment},
  author={Albarelli, Francesco and Rossi, Matteo AC and Tamascelli, Dario and Genoni, Marco G},
  journal={Quantum},
  volume={2},
  pages={110},
  year={2018},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{burgarth2015quantum,
  title={Quantum estimation via sequential measurements},
  author={Burgarth, Daniel and Giovannetti, Vittorio and Kato, Airi N and Yuasa, Kazuya},
  journal={New Journal of Physics},
  volume={17},
  number={11},
  pages={113055},
  year={2015},
  publisher={IOP Publishing}
}

@article{catana2015fisher,
  title={Fisher informations and local asymptotic normality for continuous-time quantum Markov processes},
  author={Catana, Catalin and Bouten, Luc and Gu{\c{t}}{\u{a}}, M{\u{a}}d{\u{a}}lin},
  journal={J. Phys. A Math. Theor. },
  volume={48},
  number={36},
  pages={365301},
  year={2015},
  publisher={IOP Publishing}
}
@misc{tang2023enhancement,
      title={Enhancement of Quantum Sensing in a Cavity Optomechanical System around Quantum Critical Point}, 
      author={Tang, S.B and Qin, H. and Wang, D. Y. and  Cui, K. and Su, S. L. and Yan, L. L. and Chen, G.},
      year={2023},
      eprint={2303.16486},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{guta2017information,
  title={Information geometry and local asymptotic normality for multi-parameter estimation of quantum Markov dynamics},
  author={Guta, Madalin and Kiukas, Jukka},
  journal={Journal of Mathematical Physics},
  volume={58},
  number={5},
  pages={052201},
  year={2017},
  publisher={AIP Publishing LLC}
}


@article{ilias2022criticality,
  title = {Criticality-Enhanced Quantum Sensing via Continuous Measurement},
  author = {Ilias, Theodoros and Yang, Dayou and Huelga, Susana F. and Plenio, Martin B.},
  journal = {PRX Quantum},
  volume = {3},
  issue = {1},
  pages = {010354},
  numpages = {21},
  year = {2022},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.3.010354},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.3.010354}
}



@article{garbe2020critical,
  title = {Critical Quantum Metrology with a Finite-Component Quantum Phase Transition},
  author = {Garbe, L. and Bina, M. and Keller, A. and Paris, M. G. A. and Felicetti, S.},
  journal = {Phys. Rev. Lett.},
  volume = {124},
  issue = {12},
  pages = {120504},
  numpages = {5},
  year = {2020},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.124.120504},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.120504}
}







@article{ivanov2020enhanced,
  title={Enhanced two-parameter phase-space-displacement estimation close to a dissipative phase transition},
  author={Ivanov, Peter A},
  journal={Physical Review A},
  volume={102},
  number={5},
  pages={052611},
  year={2020},
  publisher={APS}
}






@article{shapere2012classical,
  title={Classical time crystals},
  author={Shapere, Alfred and Wilczek, Frank},
  journal={Physical review letters},
  volume={109},
  number={16},
  pages={160402},
  year={2012},
  publisher={APS}
}

@article{sacha2017time,
  title={Time crystals: a review},
  author={Sacha, Krzysztof and Zakrzewski, Jakub},
  journal={Reports on Progress in Physics},
  volume={81},
  number={1},
  pages={016401},
  year={2017},
  publisher={IOP Publishing}
}

@article{wilczek2012quantum,
  title={Quantum time crystals},
  author={Wilczek, Frank},
  journal={Physical review letters},
  volume={109},
  number={16},
  pages={160401},
  year={2012},
  publisher={APS}
}

@article{minganti2020correspondence,
  title={Correspondence between dissipative phase transitions of light and time crystals},
  author={Minganti, Fabrizio and Arkhipov, Ievgen I and Miranowicz, Adam and Nori, Franco},
  journal={arXiv preprint arXiv:2008.08075},
  year={2020}
}

@article{sieberer2016keldysh,
  title={Keldysh field theory for driven open quantum systems},
  author={Sieberer, Lukas M and Buchhold, Michael and Diehl, Sebastian},
  journal={Reports on Progress in Physics},
  volume={79},
  number={9},
  pages={096001},
  year={2016},
  publisher={IOP Publishing}
}

@article{minganti2018spectral,
  title={Spectral theory of Liouvillians for dissipative phase transitions},
  author={Minganti, Fabrizio and Biella, Alberto and Bartolo, Nicola and Ciuti, Cristiano},
  journal={Physical Review A},
  volume={98},
  number={4},
  pages={042118},
  year={2018},
  publisher={APS}
}

@article{lledo2019driven,
  title={Driven Bose-Hubbard dimer under nonlocal dissipation: A bistable time crystal},
  author={Lled{\'o}, Crist{\'o}bal and Mavrogordatos, Th K and Szyma{\'n}ska, MH},
  journal={Physical Review B},
  volume={100},
  number={5},
  pages={054303},
  year={2019},
  publisher={APS}
}

@article{li2012space,
  title={Space-time crystals of trapped ions},
  author={Li, Tongcang and Gong, Zhe-Xuan and Yin, Zhang-Qi and Quan, HT and Yin, Xiaobo and Zhang, Peng and Duan, L-M and Zhang, Xiang},
  journal={Physical review letters},
  volume={109},
  number={16},
  pages={163001},
  year={2012},
  publisher={APS}
}




@article{Agarwal1977,
  title = {Collective atomic effects in resonance fluorescence},
  author = {Agarwal, G. S. and Brown, A. C. and Narducci, L. M. and Vetri, G.},
  journal = {Phys. Rev. A},
  volume = {15},
  issue = {4},
  pages = {1613--1624},
  numpages = {0},
  year = {1977},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.15.1613},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.15.1613}
}

@article{Carmichael1977,
doi = {10.1088/0022-3700/10/18/002},
url = {https://dx.doi.org/10.1088/0022-3700/10/18/002},
year = {1977},
month = {dec},
publisher = {},
volume = {10},
number = {18},
pages = {L685},
author = {H J Carmichael and  D F Walls},
title = {Hysteresis in the spectrum for cooperative resonance fluorescence},
journal = {Journal of Physics B: Atomic and Molecular Physics}
}

@article{Carmichael1980,
doi = {10.1088/0022-3700/13/18/009},
url = {https://dx.doi.org/10.1088/0022-3700/13/18/009},
year = {1980},
month = {sep},
publisher = {},
volume = {13},
number = {18},
pages = {3551},
author = {H J Carmichael},
title = {Analytical and numerical results for the steady state in cooperative resonance fluorescence},
journal = {Journal of Physics B: Atomic and Molecular Physics}
}

@article{Walls1980,
doi = {10.1088/0022-3700/13/10/008},
url = {https://dx.doi.org/10.1088/0022-3700/13/10/008},
year = {1980},
month = {may},
publisher = {},
volume = {13},
number = {10},
pages = {2001},
author = {D F Walls},
title = {Cooperative fluorescence from N coherently driven two-level atoms},
journal = {Journal of Physics B: Atomic and Molecular Physics}
}

@article{Walls1978,
	Author = {Walls, D. F. and Drummond, P. D. and Hassan, S. S. and Carmichael, H. J.},
	Doi = {10.1143/PTPS.64.307},
	Issn = {0375-9687},
	Journal = {Progress of Theoretical Physics Supplement},
	Month = {02},
	Pages = {307-320},
	Title = {{Non-Equilibrium Phase Transitions in Cooperative Atomic Systems}},
	Url = {https://doi.org/10.1143/PTPS.64.307},
	Volume = {64},
	Year = {1978},
	Bdsk-Url-1 = {https://doi.org/10.1143/PTPS.64.307}}

@article{Carmichael1980,
doi = {10.1088/0022-3700/13/18/009},
url = {https://dx.doi.org/10.1088/0022-3700/13/18/009},
year = {1980},
month = {sep},
publisher = {},
volume = {13},
number = {18},
pages = {3551},
author = {H J Carmichael},
title = {Analytical and numerical results for the steady state in cooperative resonance fluorescence},
journal = {Journal of Physics B: Atomic and Molecular Physics}}

@article{morrison2008dissipation,
  title={Dissipation-driven quantum phase transitions in collective spin systems},
  author={Morrison, S and Parkins, AS},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={41},
  number={19},
  pages={195502},
  year={2008},
  publisher={IOP Publishing}
}

@article{ferioli2022observation,
  title={Observation of a non-equilibrium superradiant phase transition in free space},
  author={Ferioli, Giovanni and Glicenstein, Antoine and Ferrier-Barbut, Igor and Browaeys, Antoine},
  journal={arXiv preprint arXiv:2207.10361},
  year={2022}
}

@article{iemini2018boundary,
  title={Boundary time crystals},
  author={Iemini, F and Russomanno, A and Keeling, J and Schir{\`o}, M and Dalmonte, M and Fazio, R},
  journal={Physical review letters},
  volume={121},
  number={3},
  pages={035301},
  year={2018},
  publisher={APS}
}

@article{carollo2022exact,
  title={Exact solution of a boundary time-crystal phase transition: time-translation symmetry breaking and non-Markovian dynamics of correlations},
  author={Carollo, Federico and Lesanovsky, Igor},
  journal={Physical Review A},
  volume={105},
  number={4},
  pages={L040202},
  year={2022},
  publisher={APS}
}

@article{lledo2020dissipative,
  title={A dissipative time crystal with or without Z2 symmetry breaking},
  author={Lled{\'o}, Crist{\'o}bal and Szyma{\'n}ska, Marzena H},
  journal={New Journal of Physics},
  volume={22},
  number={7},
  pages={075002},
  year={2020},
  publisher={IOP Publishing}
}

@article{sakurai2021chimera,
  title={Chimera Time-Crystalline order in quantum spin networks},
  author={Sakurai, A and Bastidas, VM and Munro, WJ and Nemoto, Kae},
  journal={Physical Review Letters},
  volume={126},
  number={12},
  pages={120606},
  year={2021},
  publisher={APS}
}

@article{else2016floquet,
  title={Floquet time crystals},
  author={Else, Dominic V and Bauer, Bela and Nayak, Chetan},
  journal={Physical review letters},
  volume={117},
  number={9},
  pages={090402},
  year={2016},
  publisher={APS}
}

@article{guo2020condensed,
  title={Condensed matter physics in time crystals},
  author={Guo, Lingzhen and Liang, Pengfei},
  journal={New Journal of Physics},
  volume={22},
  number={7},
  pages={075003},
  year={2020},
  publisher={IOP Publishing}
}

@article{russomanno2017floquet,
  title={Floquet time crystal in the Lipkin-Meshkov-Glick model},
  author={Russomanno, Angelo and Iemini, Fernando and Dalmonte, Marcello and Fazio, Rosario},
  journal={Physical Review B},
  volume={95},
  number={21},
  pages={214307},
  year={2017},
  publisher={APS}
}

@article{pizzi2021higher,
  title={Higher-order and fractional discrete time crystals in clean long-range interacting systems},
  author={Pizzi, Andrea and Knolle, Johannes and Nunnenkamp, Andreas},
  journal={Nature communications},
  volume={12},
  number={1},
  pages={1--7},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{surace2019floquet,
  title={Floquet time crystals in clock models},
  author={Surace, Federica Maria and Russomanno, Angelo and Dalmonte, Marcello and Silva, Alessandro and Fazio, Rosario and Iemini, Fernando},
  journal={Physical Review B},
  volume={99},
  number={10},
  pages={104303},
  year={2019},
  publisher={APS}
}

@article{gambetta2019discrete,
  title={Discrete time crystals in the absence of manifest symmetries or disorder in open quantum systems},
  author={Gambetta, FM and Carollo, F and Marcuzzi, M and Garrahan, JP and Lesanovsky, I},
  journal={Physical review letters},
  volume={122},
  number={1},
  pages={015701},
  year={2019},
  publisher={APS}
}

@article{riera2020time,
  title={Time crystallinity in open quantum systems},
  author={Riera-Campeny, Andreu and Moreno-Cardoner, Maria and Sanpera, Anna},
  journal={Quantum},
  volume={4},
  pages={270},
  year={2020},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{estarellas2020simulating,
  title={Simulating complex quantum networks with time crystals},
  author={Estarellas, MP and Osada, T and Bastidas, VM and Renoust, Benjamin and Sanaka, K and Munro, WJ and Nemoto, K},
  journal={Science advances},
  volume={6},
  number={42},
  pages={eaay8892},
  year={2020},
  publisher={American Association for the Advancement of Science}
}

@article{mi2022time,
  title={Time-crystalline eigenstate order on a quantum processor},
  author={Mi, Xiao and Ippoliti, Matteo and Quintana, Chris and Greene, Ami and Chen, Zijun and Gross, Jonathan and Arute, Frank and Arya, Kunal and Atalaya, Juan and Babbush, Ryan and others},
  journal={Nature},
  volume={601},
  number={7894},
  pages={531--536},
  year={2022},
  publisher={Nature Publishing Group}
}

@article{rovny2018observation,
  title={Observation of discrete-time-crystal signatures in an ordered dipolar many-body system},
  author={Rovny, Jared and Blum, Robert L and Barrett, Sean E},
  journal={Physical review letters},
  volume={120},
  number={18},
  pages={180603},
  year={2018},
  publisher={APS}
}

@article{smits2018observation,
  title={Observation of a space-time crystal in a superfluid quantum gas},
  author={Smits, Jasper and Liao, Lei and Stoof, HTC and van der Straten, Peter},
  journal={Physical review letters},
  volume={121},
  number={18},
  pages={185301},
  year={2018},
  publisher={APS}
}

@article{pal2018temporal,
  title={Temporal order in periodically driven spins in star-shaped clusters},
  author={Pal, Soham and Nishad, Naveen and Mahesh, TS and Sreejith, GJ},
  journal={Physical review letters},
  volume={120},
  number={18},
  pages={180602},
  year={2018},
  publisher={APS}
}

@article{pal2018temporal,
  title={Temporal order in periodically driven spins in star-shaped clusters},
  author={Pal, Soham and Nishad, Naveen and Mahesh, TS and Sreejith, GJ},
  journal={Physical review letters},
  volume={120},
  number={18},
  pages={180602},
  year={2018},
  publisher={APS}
}


@article{choi2017observation,
  title={Observation of discrete time-crystalline order in a disordered dipolar many-body system},
  author={Choi, Soonwon and Choi, Joonhee and Landig, Renate and Kucsko, Georg and Zhou, Hengyun and Isoya, Junichi and Jelezko, Fedor and Onoda, Shinobu and Sumiya, Hitoshi and Khemani, Vedika and others},
  journal={Nature},
  volume={543},
  number={7644},
  pages={221--225},
  year={2017},
  publisher={Nature Publishing Group}
}


@article{zhang2017observation,
  title={Observation of a discrete time crystal},
  author={Zhang, Jiehang and Hess, Paul W and Kyprianidis, A and Becker, Petra and Lee, A and Smith, J and Pagano, Gaetano and Potirniche, I-D and Potter, Andrew C and Vishwanath, Ashvin and others},
  journal={Nature},
  volume={543},
  number={7644},
  pages={217--220},
  year={2017},
  publisher={Nature Publishing Group}
}


@article{li2012space,
  title={Space-time crystals of trapped ions},
  author={Li, Tongcang and Gong, Zhe-Xuan and Yin, Zhang-Qi and Quan, HT and Yin, Xiaobo and Zhang, Peng and Duan, L-M and Zhang, Xiang},
  journal={Physical review letters},
  volume={109},
  number={16},
  pages={163001},
  year={2012},
  publisher={APS}
}


@article{cabot2022quantum,
  title={Quantum trajectories of dissipative time-crystals},
  author={Cabot, Albert and Muhle, Leah Sophie and Carollo, Federico and Lesanovsky, Igor},
  journal={arXiv preprint arXiv:2212.06460},
  year={2022}
}

@article{kolodynski2013efficient,
  title={Efficient tools for quantum metrology with uncorrelated noise},
  author={Ko{\l}ody{\'n}ski, Jan and Demkowicz-Dobrza{\'n}ski, Rafa{\l}},
  journal={New Journal of Physics},
  volume={15},
  number={7},
  pages={073043},
  year={2013},
  publisher={IOP Publishing}
}

@article{skotiniotis2015quantum,
  title={Quantum metrology for the Ising Hamiltonian with transverse magnetic field},
  author={Skotiniotis, Michael and Sekatski, Pavel and D{\"u}r, Wolfgang},
  journal={New Journal of Physics},
  volume={17},
  number={7},
  pages={073032},
  year={2015},
  publisher={IOP Publishing}
}

@article{de2013quantum,
  title = {Quantum parameter estimation affected by unitary disturbance},
  author = {De Pasquale, A. and Rossini, D. and Facchi, P. and Giovannetti, V.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {5},
  pages = {052117},
  numpages = {5},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.052117},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.052117}
}


@article{boixo2007generalized,
  title={Generalized limits for single-parameter quantum estimation},
  author={Boixo, Sergio and Flammia, Steven T and Caves, Carlton M and Geremia, John M},
  journal={Physical review letters},
  volume={98},
  number={9},
  pages={090401},
  year={2007},
  publisher={APS}
}

@article{pang2014quantum,
  title={Quantum metrology for a general Hamiltonian parameter},
  author={Pang, Shengshi and Brun, Todd A},
  journal={Physical Review A},
  volume={90},
  number={2},
  pages={022117},
  year={2014},
  publisher={APS}
}


@article{bayat2017scaling,
  title={Scaling of tripartite entanglement at impurity quantum phase transitions},
  author={Bayat, Abolfazl},
  journal={Phys. Rev. Lett.},
  volume={118},
  number={3},
  pages={036102},
  year={2017},
  publisher={APS}
}

@article{burgarth2014exponential,
  title={Exponential rise of dynamical complexity in quantum computing through projections},
  author={Burgarth, Daniel Klaus and Facchi, Paolo and Giovannetti, Vittorio and Nakazato, Hiromichi and Pascazio, Saverio and Yuasa, Kazuya},
  journal={Nat. Commun.},
  volume={5},
  number={1},
  pages={1--6},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{pouyandeh2014measurement,
  title={Measurement-induced dynamics for spin-chain quantum communication and its application for optical lattices},
  author={Pouyandeh, Sima and Shahbazi, Farhad and Bayat, Abolfazl},
  journal={Phys. Rev. A},
  volume={90},
  number={1},
  pages={012337},
  year={2014},
  publisher={APS}
}

@article{ma2018phase,
  title={Phase transitions in sequential weak measurements},
  author={Ma, Wen-Long and Wang, Ping and Leong, Weng-Hang and Liu, Ren-Bao},
  journal={Physical Review A},
  volume={98},
  number={1},
  pages={012117},
  year={2018},
  publisher={APS}
}

@article{bayat2018measurement,
  title={Measurement quench in many-body systems},
  author={Bayat, Abolfazl and Alkurtass, Bedoor and Sodano, Pasquale and Johannesson, Henrik and Bose, Sougato},
  journal={Physical Review Letters},
  volume={121},
  number={3},
  pages={030601},
  year={2018},
  publisher={APS}
}




@article{skinner2019measurement,
  title={Measurement-induced phase transitions in the dynamics of entanglement},
  author={Skinner, Brian and Ruhman, Jonathan and Nahum, Adam},
  journal={Physical Review X},
  volume={9},
  number={3},
  pages={031009},
  year={2019},
  publisher={APS}
}

@article{feng2022measurement,
  title={Measurement-induced phase transitions on dynamical quantum trees},
  author={Feng, Xiaozhou and Skinner, Brian and Nahum, Adam},
  journal={arXiv preprint arXiv:2210.07264},
  year={2022}
}

@article{choi2020quantum,
  title={Quantum error correction in scrambling dynamics and measurement-induced phase transition},
  author={Choi, Soonwon and Bao, Yimu and Qi, Xiao-Liang and Altman, Ehud},
  journal={Physical Review Letters},
  volume={125},
  number={3},
  pages={030505},
  year={2020},
  publisher={APS}
}

@article{carollo2018uhlmann,
  title={Uhlmann curvature in dissipative phase transitions},
  author={Carollo, A. and Spagnolo, B. and Valenti, D.},
  journal={Sci. Rep.},
  volume={8},
  number={1},
  pages={9852},
  year={2018},
  publisher={Nature Publishing Group UK London},
  doi = {10.1038/s41598-018-27362-9},
  url = {https://doi.org/10.1038/s41598-018-27362-9}
}

@article{minato2022fate,
  title={Fate of measurement-induced phase transition in long-range interactions},
  author={Minato, Takaaki and Sugimoto, Koudai and Kuwahara, Tomotaka and Saito, Keiji},
  journal={Physical review letters},
  volume={128},
  number={1},
  pages={010603},
  year={2022},
  publisher={APS}
}

@article{gullans2020dynamical,
  title={Dynamical purification phase transition induced by quantum measurements},
  author={Gullans, Michael J and Huse, David A},
  journal={Physical Review X},
  volume={10},
  number={4},
  pages={041020},
  year={2020},
  publisher={APS}
}

@article{block2022measurement,
  title={Measurement-induced transition in long-range interacting quantum circuits},
  author={Block, Maxwell and Bao, Yimu and Choi, Soonwon and Altman, Ehud and Yao, Norman Y},
  journal={Physical Review Letters},
  volume={128},
  number={1},
  pages={010604},
  year={2022},
  publisher={APS}
}

@article{burgarth2015quantum,
  title={Quantum estimation via sequential measurements},
  author={Burgarth, Daniel and Giovannetti, Vittorio and Kato, Airi N and Yuasa, Kazuya},
  journal={New Journal of Physics},
  volume={17},
  number={11},
  pages={113055},
  year={2015},
  publisher={IOP Publishing}
}

@article{montenegro2022sequential,
  title = {Sequential Measurements for Quantum-Enhanced Magnetometry in Spin Chain Probes},
  author = {Montenegro, V. and Jones, G. S. and Bose, S. and Bayat, A.},
  journal = {Phys. Rev. Lett.},
  volume = {129},
  issue = {12},
  pages = {120503},
  numpages = {7},
  year = {2022},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.129.120503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.129.120503}
}

@article{Gietka2021adiabaticcritical,
  doi = {10.22331/q-2021-07-01-489},
  url = {https://doi.org/10.22331/q-2021-07-01-489},
  title = {Adiabatic critical quantum metrology cannot reach the {H}eisenberg limit even when shortcuts to adiabaticity are applied},
  author = {Gietka, K. and Metz, F. and Keller, T. and Li, J.},
  journal = {{Quantum}},
  issn = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {5},
  pages = {489},
  month = jul,
  year = {2021}
}

@article{PhysRevX.8.021022,
  title = {At the Limits of Criticality-Based Quantum Metrology: Apparent Super-{H}eisenberg Scaling Revisited},
  author = {Rams, M. M. and Sierant, P. and Dutta, O. and Horodecki, P/ and Zakrzewski, J.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {2},
  pages = {021022},
  numpages = {16},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.021022},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.021022}
}



@article{guta2017information,
  title={Information geometry and local asymptotic normality for multi-parameter estimation of quantum Markov dynamics},
  author={Guta, Madalin and Kiukas, Jukka},
  journal={Journal of Mathematical Physics},
  volume={58},
  number={5},
  pages={052201},
  year={2017},
  publisher={AIP Publishing LLC}
}

@article{catana2015fisher,
  title={Fisher informations and local asymptotic normality for continuous-time quantum Markov processes},
  author={Catana, Catalin and Bouten, Luc and Gu{\c{t}}{\u{a}}, M{\u{a}}d{\u{a}}lin},
  journal={J. Phys. A Math. Theor. },
  volume={48},
  number={36},
  pages={365301},
  year={2015},
  publisher={IOP Publishing}
}


@misc{mael2022,
  author = {Bompais, Maël and Amini, Nina H. and Pellegrini, Clément},
  eprint={2204.00343},
  archivePrefix={arXiv},
  primaryClass={quant-ph}
}

@INPROCEEDINGS{7403443,
  author={Six, P. and Campagne-Ibarcq, Ph. and Bretheau, L. and Huard, B. and Rouchon, P.},
  booktitle={2015 54th IEEE Conference on Decision and Control (CDC)}, 
  title={Parameter estimation from measurements along quantum trajectories}, 
  year={2015},
  volume={},
  number={},
  pages={7742-7748},
  doi={10.1109/CDC.2015.7403443}}


@article{cuatanua2012asymptotic,
  title={Asymptotic inference in system identification for the atom maser},
  author={C{\u{a}}tan{\u{a}}, C{\u{a}}t{\u{a}}lin and van Horssen, Merlijn and Gu{\c{t}}{\u{a}}, M{\u{a}}d{\u{a}}lin},
  journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={370},
  number={1979},
  pages={5308--5323},
  year={2012},
  publisher={The Royal Society Publishing}
}

@article{guctua2011fisher,
  title={Fisher information and asymptotic normality in system identification for quantum Markov chains},
  author={Gu{\c{t}}{\u{a}}, M{\u{a}}d{\u{a}}lin},
  journal={Physical Review A},
  volume={83},
  number={6},
  pages={062324},
  year={2011},
  publisher={APS}
}

@article{de2017estimating,
  title={Estimating temperature via sequential measurements},
  author={De Pasquale, Antonella and Yuasa, Kazuya and Giovannetti, Vittorio},
  journal={Physical Review A},
  volume={96},
  number={1},
  pages={012316},
  year={2017},
  publisher={APS}
}

@article{mabuchi1996dynamical,
  title={Dynamical identification of open quantum systems},
  author={Mabuchi, Hideo},
  journal={Quantum and Semiclassical Optics: Journal of the European Optical Society Part B},
  volume={8},
  number={6},
  pages={1103},
  year={1996},
  publisher={IOP Publishing}
}
@article{gambetta2001state,
  title={State and dynamical parameter estimation for open quantum systems},
  author={Gambetta, Jay and Wiseman, Howard Mark},
  journal={Physical Review A},
  volume={64},
  number={4},
  pages={042105},
  year={2001},
  publisher={APS}
}


@article{van2015sanov,
  title={Sanov and central limit theorems for output statistics of quantum Markov chains},
  author={van Horssen, Merlijn and Gu{\c{t}}{\u{a}}, M{\u{a}}d{\u{a}}lin},
  journal={Journal of Mathematical Physics},
  volume={56},
  number={2},
  pages={022109},
  year={2015},
  publisher={AIP Publishing LLC}
}

@article{clark2019quantum,
  title={Quantum jump metrology},
  author={Clark, Lewis A and Stokes, Adam and Beige, Almut},
  journal={Physical Review A},
  volume={99},
  number={2},
  pages={022102},
  year={2019},
  publisher={APS}
}

@article{rasbi2022jumps,
  title = {Quantum jump metrology in a two-cavity network},
  author = {Rasbi, Kawthar Al and Beige, Almut and Clark, Lewis A.},
  journal = {Phys. Rev. A},
  volume = {106},
  issue = {6},
  pages = {062619},
  numpages = {12},
  year = {2022},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.106.062619},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.106.062619}
}


@article{brennecke2013real,
  title={Real-time observation of fluctuations at the driven-dissipative Dicke phase transition},
  author={Brennecke, Ferdinand and Mottl, Rafael and Baumann, Kristian and Landig, Renate and Donner, Tobias and Esslinger, Tilman},
  journal={Proceedings of the National Academy of Sciences},
  volume={110},
  number={29},
  pages={11763--11767},
  year={2013},
  publisher={National Acad Sciences}
}

@article{fitzpatrick2017observation,
  title={Observation of a dissipative phase transition in a one-dimensional circuit QED lattice},
  author={Fitzpatrick, Mattias and Sundaresan, Neereja M and Li, Andy CY and Koch, Jens and Houck, Andrew A},
  journal={Physical Review X},
  volume={7},
  number={1},
  pages={011016},
  year={2017},
  publisher={APS}
}

@article{ferri2021emerging,
  title={Emerging dissipative phases in a superradiant quantum gas with tunable decay},
  author={Ferri, Francesco and Rosa-Medina, Rodrigo and Finger, Fabian and Dogra, Nishant and Soriente, Matteo and Zilberberg, Oded and Donner, Tobias and Esslinger, Tilman},
  journal={Physical Review X},
  volume={11},
  number={4},
  pages={041046},
  year={2021},
  publisher={APS}
}

@article{cai2022probing,
  title={Probing a dissipative phase transition with a trapped ion through reservoir engineering},
  author={Cai, M-L and Liu, Z-D and Jiang, Y and Wu, Y-K and Mei, Q-X and Zhao, W-D and He, L and Zhang, X and Zhou, Z-C and Duan, L-M},
  journal={Chinese Physics Letters},
  volume={39},
  number={2},
  pages={020502},
  year={2022},
  publisher={IOP Publishing}
}

@article{fink2018signatures,
  title={Signatures of a dissipative phase transition in photon correlation measurements},
  author={Fink, Thomas and Schade, Anne and H{\"o}fling, Sven and Schneider, Christian and Imamoglu, Ata{\c{c}}},
  journal={Nature Physics},
  volume={14},
  number={4},
  pages={365--369},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{ohadi2015spontaneous,
  title={Spontaneous spin bifurcations and ferromagnetic phase transitions in a spinor exciton-polariton condensate},
  author={Ohadi, Hamid and Dreismann, A and Rubo, YG and Pinsker, F and Redondo, Y del Valle-Inclan and Tsintzos, SI and Hatzopoulos, Z and Savvidis, PG and Baumberg, JJ},
  journal={Physical Review X},
  volume={5},
  number={3},
  pages={031002},
  year={2015},
  publisher={APS}
}
@article{bin2019mass,
  title={Mass sensing by quantum criticality},
  author={Bin, S.W. and L{\"u}, X.Y. and Yin, T.S. and Zhu, G.L. and Bin, Q. and Wu, Y.},
  journal={Optics Letters},
  volume={44},
  number={3},
  pages={630--633},
  year={2019},
  publisher={Optica Publishing Group},
  doi = {10.1364/OL.44.000630},
  url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-44-3-630}
}

@article{wang2019Heisenberg,
  title={{H}eisenberg-limited single-mode quantum metrology in a superconducting circuit},
  author={Wang, Weiting and Wu, Yukai and Ma, Yuwei and Cai, Weizhou and Hu, Ling and Mu, Xianghao and Xu, Yuan and Chen, Zi-Jie and Wang, Haiyan and Song, YP and others},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={4382},
  year={2019},
  publisher={Nature Publishing Group UK London}
}
@article{ding2022enhanced,
  title={Enhanced metrology at the critical point of a many-body {R}ydberg atomic system},
  author={Ding, D. S. and Liu, Z. K. and Shi, B. S. and Guo, G. C. and M{\o}lmer, K. and Adams, C. S.},
  journal={Nature Physics},
  volume={18},
  number={12},
  pages={1447--1452},
  year={2022},
  publisher={Nature Publishing Group UK London},
  doi = {10.1038/s41567-022-01777-8},
  url = {https://doi.org/10.1038/s41567-022-01777-8}
}

@article{kessler2012dissipative,
  title={Dissipative phase transition in a central spin system},
  author={Kessler, Eric M and Giedke, Geza and Imamoglu, Atac and Yelin, Susanne F and Lukin, Mikhail D and Cirac, J Ignacio},
  journal={Physical Review A},
  volume={86},
  number={1},
  pages={012116},
  year={2012},
  publisher={APS}
}

@article{ding2016phase,
  title={Phase diagram and self-organising dynamics in a strongly-interacting thermal {R}ydberg ensemble},
  author={Ding, Dong-Sheng and Busche, Hannes and Shi, Bao-Sen and Guo, Guang-Can and Adams, Charles S},
  journal={arXiv preprint arXiv:1606.08791},
  year={2016}
}

@article{collodo2019observation,
  title={Observation of the crossover from photon ordering to delocalization in tunably coupled resonators},
  author={Collodo, Michele C and Poto{\v{c}}nik, Anton and Gasparinetti, Simone and Besse, Jean-Claude and Pechal, Marek and Sameti, Mahdi and Hartmann, Michael J and Wallraff, Andreas and Eichler, Christopher},
  journal={Physical Review Letters},
  volume={122},
  number={18},
  pages={183601},
  year={2019},
  publisher={APS}
}

@article{jin2021determination,
  title={Determination of the critical exponents in dissipative phase transitions: Coherent anomaly approach},
  author={Jin, Jiasen and He, Wen-Bin and Iemini, Fernando and Ferreira, Diego and Wang, Ying-Dan and Chesi, Stefano and Fazio, Rosario},
  journal={Physical Review B},
  volume={104},
  number={21},
  pages={214301},
  year={2021},
  publisher={APS}
}

@article{carollo2019critical,
  title={Critical behavior of the quantum contact process in one dimension},
  author={Carollo, Federico and Gillman, Edward and Weimer, Hendrik and Lesanovsky, Igor},
  journal={Physical Review Letters},
  volume={123},
  number={10},
  pages={100604},
  year={2019},
  publisher={APS}
}

@article{maghrebi2016nonequilibrium,
  title={Nonequilibrium many-body steady states via Keldysh formalism},
  author={Maghrebi, Mohammad F and Gorshkov, Alexey V},
  journal={Physical Review B},
  volume={93},
  number={1},
  pages={014307},
  year={2016},
  publisher={APS}
}

@article{marino2016driven,
  title={Driven markovian quantum criticality},
  author={Marino, Jamir and Diehl, Sebastian},
  journal={Physical review letters},
  volume={116},
  number={7},
  pages={070407},
  year={2016},
  publisher={APS}
}

@article{sieberer2013dynamical,
  title={Dynamical critical phenomena in driven-dissipative systems},
  author={Sieberer, LM and Huber, Sebastian D and Altman, Ehud and Diehl, S},
  journal={Physical review letters},
  volume={110},
  number={19},
  pages={195301},
  year={2013},
  publisher={APS}
}

@article{marcuzzi2014universal,
  title={Universal nonequilibrium properties of dissipative {R}ydberg gases},
  author={Marcuzzi, Matteo and Levi, Emanuele and Diehl, Sebastian and Garrahan, Juan P and Lesanovsky, Igor},
  journal={Physical review letters},
  volume={113},
  number={21},
  pages={210401},
  year={2014},
  publisher={APS}
}

@article{overbeck2017multicritical,
  title={Multicritical behavior in dissipative Ising models},
  author={Overbeck, Vincent R and Maghrebi, Mohammad F and Gorshkov, Alexey V and Weimer, Hendrik},
  journal={Physical Review A},
  volume={95},
  number={4},
  pages={042133},
  year={2017},
  publisher={APS}
}

@article{casteels2017critical,
  title={Critical dynamical properties of a first-order dissipative phase transition},
  author={Casteels, Wim and Fazio, Rosario and Ciuti, Christiano},
  journal={Physical Review A},
  volume={95},
  number={1},
  pages={012128},
  year={2017},
  publisher={APS}
}

@article{vicentini2018critical,
  title={Critical slowing down in driven-dissipative Bose-Hubbard lattices},
  author={Vicentini, Filippo and Minganti, Fabrizio and Rota, Riccardo and Orso, Giuliano and Ciuti, Cristiano},
  journal={Physical Review A},
  volume={97},
  number={1},
  pages={013853},
  year={2018},
  publisher={APS}
}

@article{casteels2016power,
  title={Power laws in the dynamic hysteresis of quantum nonlinear photonic resonators},
  author={Casteels, Wim and Storme, Florent and Le Boit{\'e}, Alexandre and Ciuti, Cristiano},
  journal={Physical Review A},
  volume={93},
  number={3},
  pages={033824},
  year={2016},
  publisher={APS}
}

@article{letscher2016bistability,
  title={Bistability vs. metastability in driven dissipative {R}ydberg gases},
  author={Letscher, Fabian and Thomas, Oliver and Niederpr{\"u}m, Thomas and Fleischhauer, Michael and Ott, Herwig},
  journal={arXiv preprint arXiv:1611.00627},
  year={2016}
}

@article{raghunandan2018high,
  title={High-density quantum sensing with dissipative first order transitions},
  author={Raghunandan, Meghana and Wrachtrup, J{\"o}rg and Weimer, Hendrik},
  journal={Physical Review Letters},
  volume={120},
  number={15},
  pages={150501},
  year={2018},
  publisher={APS}
}

@article{benary2022experimental,
  title={Experimental observation of a dissipative phase transition in a multi-mode many-body quantum system},
  author={Benary, Jens and Baals, Christian and Bernhart, Erik and Jiang, Jian and R{\"o}hrle, Marvin and Ott, Herwig},
  journal={arXiv preprint arXiv:2203.09896},
  year={2022}
}
@article{lourencco2022genuine,
  title={Genuine multipartite correlations in a boundary time crystal},
  author={Louren{\c{c}}o, Ant{\^o}nio C and dos Prazeres, Luis Fernando and Maciel, Thiago O and Iemini, Fernando and Duzzioni, Eduardo I},
  journal={Physical Review B},
  volume={105},
  number={13},
  pages={134422},
  year={2022},
  publisher={APS}
}

@article{montenegro2023quantum,
  title={Quantum-Enhanced Boundary Time Crystal Sensors},
  author={Montenegro, V and Genoni, MG and Bayat, A and Paris, MGA},
  journal={arXiv preprint arXiv:2301.02103},
  year={2023}
}



@article{albuquerque2010quantum,
  title = {Quantum critical scaling of fidelity susceptibility},
  author = {Albuquerque, A. F. and Alet, F. and Sire, C. and Capponi, S.},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {6},
  pages = {064418},
  numpages = {12},
  year = {2010},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.064418},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.064418}
}




@article{albarelli2018restoring,
  title={Restoring {H}eisenberg scaling in noisy quantum metrology by monitoring the environment},
  author={Albarelli, Francesco and Rossi, Matteo AC and Tamascelli, Dario and Genoni, Marco G},
  journal={Quantum},
  volume={2},
  pages={110},
  year={2018},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}


@article{rossi2020noisy,
  title={Noisy quantum metrology enhanced by continuous nondemolition measurement},
  author={Rossi, Matteo AC and Albarelli, Francesco and Tamascelli, Dario and Genoni, Marco G},
  journal={Phys. Rev. Lett.},
  volume={125},
  number={20},
  pages={200505},
  year={2020},
  publisher={APS}
}

@article{chin2012quantum,
  title={Quantum metrology in non-Markovian environments},
  author={Chin, Alex W and Huelga, Susana F and Plenio, Martin B},
  journal={Phys. Rev. Lett.},
  volume={109},
  number={23},
  pages={233601},
  year={2012},
  publisher={APS}
}

@article{chaves2013noisy,
  title={Noisy metrology beyond the standard quantum limit},
  author={Chaves, R and Brask, JB and Markiewicz, Marcin and Ko{\l}ody{\'n}ski, J and Ac{\'\i}n, A},
  journal={Physical review letters},
  volume={111},
  number={12},
  pages={120401},
  year={2013},
  publisher={APS}
}

@article{brask2015improved,
  title={Improved quantum magnetometry beyond the standard quantum limit},
  author={Brask, Jonatan Bohr and Chaves, Rafael and Ko{\l}ody{\'n}ski, Jan},
  journal={Phys. Rev. X},
  volume={5},
  number={3},
  pages={031010},
  year={2015},
  publisher={APS}
}


@article{smirne2016ultimate,
  title={Ultimate precision limits for noisy frequency estimation},
  author={Smirne, Andrea and Ko{\l}ody{\'n}ski, Jan and Huelga, Susana F and Demkowicz-Dobrza{\'n}ski, Rafa{\l}},
  journal={Physical review letters},
  volume={116},
  number={12},
  pages={120801},
  year={2016},
  publisher={APS}
}
@article{lorenzo2017quantum,
  title = {Quantum sensing close to a dissipative phase transition: Symmetry breaking and criticality as metrological resources},
  author = {Fern\'andez-Lorenzo, S. and Porras, D.},
  journal = {Phys. Rev. A},
  volume = {96},
  issue = {1},
  pages = {013817},
  numpages = {10},
  year = {2017},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.96.013817},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.96.013817}
}

@article{Garbe2022critical,
doi = {10.1088/2058-9565/ac6ca5},
url = {https://dx.doi.org/10.1088/2058-9565/ac6ca5},
year = {2022},
month = {may},
publisher = {IOP Publishing},
volume = {7},
number = {3},
pages = {035010},
author = {Garbe, L. and Abah, O. and Felicetti, S. and  Puebla, R.},
title = {Critical quantum metrology with fully-connected models: from {H}eisenberg to Kibble–Zurek scaling},
journal = {Quantum Sci. Technol.},
}

@article{dicandia2023critical,
   title={Critical parametric quantum sensing},
   volume={9},
   ISSN={2056-6387},
   url={http://dx.doi.org/10.1038/s41534-023-00690-z},
   doi={10.1038/s41534-023-00690-z},
   number={1},
   journal={Npj Quantum Inf.},
   publisher={Springer Science and Business Media LLC},
   author={Di Candia, R. and Minganti, F. and Petrovnin, K. V. and Paraoanu, G. S. and Felicetti, S.},
   year={2023},
   month={Mar} }

@article{mirkhalaf2021criticality,
  title = {Criticality-enhanced quantum sensing in ferromagnetic Bose-Einstein condensates: Role of readout measurement and detection noise},
  author = {Mirkhalaf, S. S. and Benedicto Orenes, D. and Mitchell, M. W. and Witkowska, E.},
  journal = {Phys. Rev. A},
  volume = {103},
  issue = {2},
  pages = {023317},
  numpages = {15},
  year = {2021},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.103.023317},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.103.023317}
}
@article{wu2021criticality,
  title = {Criticality-enhanced quantum sensor at finite temperature},
  author = {Wu, W. and Shi, C.},
  journal = {Phys. Rev. A},
  volume = {104},
  issue = {2},
  pages = {022612},
  numpages = {10},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.104.022612},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.104.022612}
}


@article{alldridge2020bulk,
  title={Bulk-boundary correspondence for disordered free-fermion topological phases},
  author={Alldridge, Alexander and Max, Christopher and Zirnbauer, Martin R},
  journal={Communications in Mathematical Physics},
  volume={377},
  number={3},
  pages={1761--1821},
  year={2020},
  publisher={Springer}
}


@book{alase2019boundary,
  title={Boundary physics and bulk-boundary correspondence in topological phases of matter},
  author={Alase, Abhijeet},
  year={2019},
  publisher={Dartmouth College}
}


@incollection{bernevig2013topological,
  title={Topological insulators and topological superconductors},
  author={Bernevig, B Andrei},
  booktitle={Topological Insulators and Topological Superconductors},
  year={2013},
  publisher={Princeton university press}
}

@article{chen2013symmetry,
  title={Symmetry protected topological orders and the group cohomology of their symmetry group},
  author={Chen, Xie and Gu, Zheng-Cheng and Liu, Zheng-Xin and Wen, Xiao-Gang},
  journal={Phys. Rev. B},
  volume={87},
  number={15},
  pages={155114},
  year={2013},
  publisher={APS}
}




@article{PhysRev.76.1269,
  title = {Experimental Study of the Compton Effect at 1.2 Mev},
  author = {Hofstadter, Robert and Mcintyre, John A.},
  journal = {Phys. Rev.},
  volume = {76},
  issue = {8},
  pages = {1269--1270},
  numpages = {0},
  year = {1949},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.76.1269},
  url = {https://link.aps.org/doi/10.1103/PhysRev.76.1269}
}


@article{PhysRevLett.115.180401,
  title = {Localization of Interacting Fermions in the Aubry-Andr\'e Model},
  author = {Mastropietro, Vieri},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {18},
  pages = {180401},
  numpages = {5},
  year = {2015},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.180401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.180401}
}

@article{mastropietro2017localization,
  title={Localization in interacting fermionic chains with quasi-random disorder},
  author={Mastropietro, Vieri},
  journal={Communications in Mathematical Physics},
  volume={351},
  number={1},
  pages={283--309},
  year={2017},
  publisher={Springer}
}
@article{su1979solitons,
  title = {Solitons in Polyacetylene},
  author = {Su, W. P. and Schrieffer, J. R. and Heeger, A. J.},
  journal = {Phys. Rev. Lett.},
  volume = {42},
  issue = {25},
  pages = {1698--1701},
  numpages = {0},
  year = {1979},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.42.1698},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.42.1698}
}


@misc{cabot2023continuous,
      title={Continuous sensing and parameter estimation with the boundary time-crystal}, 
      author={ Cabot, A. and  Carollo, F. and  Lesanovsky, I.},
      year={2023},
      eprint={2307.13277},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{derzhko2005regularly,
  title = {Regularly alternating spin-$\frac{1}{2}$ anisotropic $XY$ chains: The ground-state and thermodynamic properties},
  author = {Derzhko, Oleg and Richter, Johannes and Krokhmalskii, Taras and Zaburannyi, Oles'},
  journal = {Phys. Rev. E},
  volume = {69},
  issue = {6},
  pages = {066112},
  numpages = {13},
  year = {2004},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.69.066112},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.69.066112}
}


@article{derzhko2002quantum,
  title = {Quantum phase transitions in alternating transverse Ising chains: Analytical and numerical results},
  author = {Derzhko, Oleg and Richter, Johannes and Krokhmalskii, Taras and Zaburannyi, Oles'},
  journal = {Phys. Rev. B},
  volume = {66},
  issue = {14},
  pages = {144401},
  numpages = {5},
  year = {2002},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.66.144401},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.66.144401}
}

@inbook{derzhkobookquantum,
author = { Oleg   Derzhko },
title = {QUANTUM PHASE TRANSITIONS IN ALTERNATING TRANSVERSE ISING CHAINS},
booktitle = {Order, Disorder and Criticality},
chapter = {},
pages = {109-145},
doi = {10.1142/9789812565440_0003},
URL = {https://www.worldscientific.com/doi/abs/10.1142/9789812565440_0003},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/9789812565440_0003},
    abstract = { Abstract This chapter is devoted to a discussion of quantum phase transitions in a regularly alternating spin-½ Ising chain in a transverse field. After recalling some generally known topics of the classical (temperature-driven) phase transition theory and some basic concepts of the quantum phase transition theory I pass to the statistical mechanics calculations for a one-dimensional spin-½ Ising model in a transverse field, which is the simplest possible system exhibiting the continuous quantum phase transition. The essential tool for these calculations is the Jordan–Wigner fermionization. The latter technique being completed by the continued fraction approach enables one to obtain analytically the thermodynamic quantities for a “slightly complicated” model in which the intersite exchange interactions and on-site fields vary regularly along a chain. Rigorous analytical results for the ground-state and thermodynamic quantities, as well as exact numerical data for the spin correlations computed for long chains demonstrate how the regularly alternating bonds/fields affect the quantum phase transition. I discuss in detail the case of period 2, swiftly sketch the case of period 3 and finally summarize emphasizing the effects of periodically modulated Hamiltonian parameters on quantum phase transitions in the transverse Ising chain and in some related models. }
}
@article{PhysRevLett.119.075702,
  title = {Two Universality Classes for the Many-Body Localization Transition},
  author = {Khemani, Vedika and Sheng, D. N. and Huse, David A.},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {7},
  pages = {075702},
  numpages = {6},
  year = {2017},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.075702},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.075702}
}
@article{montenegro2023boundary,
	doi = {10.1038/s42005-023-01423-6},
  
	url = {https://doi.org/10.1038%2Fs42005-023-01423-6},
  
	year = 2023,
	month = {oct},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {6},
  
	number = {1},
  
	author = { Montenegro, V. and Genoni, M. G. and  Bayat, A. and  Paris, M. G. A.},
  
	title = {Quantum metrology with boundary time crystals},
  
	journal = {Communications Physics}
}
@Article{10.21468/SciPostPhys.1.1.010,
	title={{Detecting a many-body mobility edge with quantum quenches}},
	author={Piero Naldesi and Elisa Ercolessi and Tommaso Roscilde},
	journal={SciPost Phys.},
	volume={1},
	pages={010},
	year={2016},
	publisher={SciPost},
	doi={10.21468/SciPostPhys.1.1.010},
	url={https://scipost.org/10.21468/SciPostPhys.1.1.010},
}

@article{PhysRevB.96.104205,
  title = {Transport properties across the many-body localization transition in quasiperiodic and random systems},
  author = {Setiawan, F. and Deng, Dong-Ling and Pixley, J. H.},
  journal = {Phys. Rev. B},
  volume = {96},
  issue = {10},
  pages = {104205},
  numpages = {13},
  year = {2017},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.96.104205},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.96.104205}
}

@misc{sahoo2023localization,
      title={Localization Driven Quantum Sensing}, 
      author={ Sahoo, A. and  Mishra, U. and  Rakshit, D.},
      year={2023},
      eprint={2305.02315},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
@article{yousefjani2023floquet,
  title = {Floquet-induced localization in long-range many-body systems},
  author = {Yousefjani, Rozhin and Bose, Sougato and Bayat, Abolfazl},
  journal = {Phys. Rev. Res.},
  volume = {5},
  issue = {1},
  pages = {013094},
  numpages = {7},
  year = {2023},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.5.013094},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.013094}
}
@article{Yousefjani2023long,
	doi = {10.1088/1674-1056/acf302},
  
	url = {https://doi.org/10.1088%2F1674-1056%2Facf302},
  
	year = 2023,
	month = {oct},
  
	publisher = {{IOP} Publishing},
  
	volume = {32},
  
	number = {10},
  
	pages = {100313},
  
	author = { Yousefjani, R. and  He, X. and Bayat, A.},
  
	title = {Long-range interacting Stark many-body probes with super-{H}eisenberg precision},
  
	journal = {Chinese Physics B}
}
@article{he22023stark,
  title = {Stark Localization as a Resource for Weak-Field Sensing with Super-{H}eisenberg Precision},
  author = {He, X. and Yousefjani, R. and Bayat, A.},
  journal = {Phys. Rev. Lett.},
  volume = {131},
  issue = {1},
  pages = {010801},
  numpages = {7},
  year = {2023},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.131.010801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.131.010801}
}

@article{mishra2021driving,
  title = {Driving Enhanced Quantum Sensing in Partially Accessible Many-Body Systems},
  author = {Mishra, U. and Bayat, A.},
  journal = {Phys. Rev. Lett.},
  volume = {127},
  issue = {8},
  pages = {080504},
  numpages = {7},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.127.080504},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.127.080504}
}




@misc{zhang2023topological,
      title={Topological Waveguide Quantum Sensors}, 
      author={Zhang, T. and Hu, J. and Qiu, X.},
      year={2023},
      eprint={2311.01370},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@article{budich2020nonhermitian,
  title = {Non-Hermitian Topological Sensors},
  author = {Budich, J. C. and Bergholtz, E. J.},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  issue = {18},
  pages = {180403},
  numpages = {7},
  year = {2020},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.125.180403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.180403}
}

@article{alase2017generalization,
  title={Generalization of Bloch's theorem for arbitrary boundary conditions: Theory},
  author={Alase, Abhijeet and Cobanera, Emilio and Ortiz, Gerardo and Viola, Lorenza},
  journal={Physical Review B},
  volume={96},
  number={19},
  pages={195133},
  year={2017},
  publisher={APS}
}

@article{cobanera2018generalization,
  title={Generalization of Bloch's theorem for arbitrary boundary conditions: Interfaces and topological surface band structure},
  author={Cobanera, Emilio and Alase, Abhijeet and Ortiz, Gerardo and Viola, Lorenza},
  journal={Physical Review B},
  volume={98},
  number={24},
  pages={245423},
  year={2018},
  publisher={APS}
}


  @misc{supp,
author = {},
title = {},
howpublished = "See supplementary material",
year = {},
note = " "}

@article{montenegro2021global,
  title = {Global Sensing and Its Impact for Quantum Many-Body Probes with Criticality},
  author = {Montenegro, Victor and Mishra, Utkarsh and Bayat, Abolfazl},
  journal = {Phys. Rev. Lett.},
  volume = {126},
  issue = {20},
  pages = {200501},
  numpages = {6},
  year = {2021},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.126.200501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.126.200501}
}

@article{mok2021optimal,
  title={Optimal probes for global quantum thermometry},
  author={Mok, Wai-Keong and Bharti, Kishor and Kwek, Leong-Chuan and Bayat, Abolfazl},
  journal={Communications physics},
  volume={4},
  number={1},
  pages={62},
  year={2021},
  publisher={Nature Publishing Group UK London}
}


@article{tong2006lee,
  title = {Lee-Yang Zeros of Periodic and Quasiperiodic Anisotropic $XY$ Chains in a Transverse Field},
  author = {Tong, Peiqing and Liu, Xiaoxian},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {1},
  pages = {017201},
  numpages = {4},
  year = {2006},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.017201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.97.017201}
}
@article{tong2002quantum,
  title = {Quantum phase transitions of a quasiperiodic anisotropic $\mathrm{XY}$ chain in a transverse magnetic field},
  author = {Tong, Peiqing and Zhong, Ming},
  journal = {Phys. Rev. B},
  volume = {65},
  issue = {6},
  pages = {064421},
  numpages = {5},
  year = {2002},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.65.064421},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.65.064421}
}

@article{delima2006the,
title = {The isotropic XY model on the inhomogeneous periodic chain},
journal = {Journal of Magnetism and Magnetic Materials},
volume = {298},
number = {2},
pages = {95-121},
year = {2006},
issn = {0304-8853},
doi = {https://doi.org/10.1016/j.jmmm.2005.03.001},
url = {https://www.sciencedirect.com/science/article/pii/S0304885305003288},
author = {J.P. {de Lima} and T.F.A. Alves and L.L. Gonçalves},
keywords = {XY model, Quantum transition, Inhomogeneous chain},
abstract = {The static and dynamic properties of the isotropic XY-model (s=12) on the inhomogeneous periodic chain, composed of N segments with n different exchange interactions and magnetic moments, in a transverse field h, are obtained exactly at arbitrary temperatures. The properties are determined by introducing the generalized Jordan–Wigner transformation and by reducing the problem to a diagonalization of a finite matrix of nth order. The diagonalization procedure is discussed in detail and the critical behaviour induced by the transverse field, at T=0, is presented. The quantum transitions are determined by analyzing the behaviour of the induced magnetization, defined as (1/n)∑m=1nμm〈Sj,mz〉 where μm is the magnetic moment at site m within the segment j, as a function of the field, and the critical fields determined exactly. The dynamic correlations, 〈Sj,mz(t)Sj′,m′z(0)〉, and the dynamic susceptibility χqzz(ω) are also obtained at arbitrary temperatures. Explicit results are presented in the limit T=0, where the critical behaviour occurs, for the static susceptibility χqzz(0) as a function of the transverse field h, and for the frequency dependency of dynamic susceptibility χqzz(ω). Also in this limit, the transverse time-correlation 〈Sj,mx(t)Sj′,m′x(0)〉 and the dynamic and isothermal susceptibilities, χqxx(ω) and χTxx, are obtained for the transverse field greater or equal than the saturation field.}
}

@article{free2022sarkar,
  title = {Free-Fermionic Topological Quantum Sensors},
  author = {Sarkar, S. and Mukhopadhyay, C. and Alase, A. and Bayat, A.},
  journal = {Phys. Rev. Lett.},
  volume = {129},
  issue = {9},
  pages = {090503},
  numpages = {6},
  year = {2022},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.129.090503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.129.090503}
}

@incollection{greenberger1989going,
  title={Going beyond Bell’s theorem},
  author={Greenberger, D. M. and Horne, M. A. and Zeilinger, A.},
  booktitle={Bell’s theorem, quantum theory and conceptions of the universe},
  pages={69--72},
  year={1989},
  publisher={Springer},
  doi = {10.1007/978-94-017-0849-4_10},
  url = {https://doi.org/10.1007/978-94-017-0849-4_10}
}


@article{leibfried2004toward,
  title={Toward {H}eisenberg-limited spectroscopy with multiparticle entangled states},
  author={Leibfried, D. and Barrett, M. D. and Schaetz, T. and Britton, J. and Chiaverini, J. and Itano, W. M. and Jost, J. D. and Langer, C. and Wineland, D. J.},
  journal={Science},
  volume={304},
  number={5676},
  pages={1476--1478},
  year={2004},
  publisher={American Association for the Advancement of Science},
  doi = {10.1126/science.1097576},
  url = {https://www.science.org/doi/abs/10.1126/science.1097576}
}

















